Benchmarking for Bayesian Reinforcement Learning

In the Bayesian Reinforcement Learning (BRL) setting, agents try to maximise the collected rewards while interacting with their environment while using some prior knowledge that is accessed beforehand. Many BRL algorithms have already been proposed, but even though a few toy examples exist in the literature, there are still no extensive or rigorous benchmarks to compare them. The paper addresses this problem, and provides a new BRL comparison methodology along with the corresponding open source library. In this methodology, a comparison criterion that measures the performance of algorithms on large sets of Markov Decision Processes (MDPs) drawn from some probability distributions is defined. In order to enable the comparison of non-anytime algorithms, our methodology also includes a detailed analysis of the computation time requirement of each algorithm. Our library is released with all source code and documentation: it includes three test problems, each of which has two different prior distributions, and seven state-of-the-art RL algorithms. Finally, our library is illustrated by comparing all the available algorithms and the results are discussed.

==> data/table-accurate-0.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{31.12 \pm 0.9}$\\
	\textbf{e-Greedy (e = 0, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{40.62 \pm 1.55}$\\
	e-Greedy (e = 0.1, GC) & $\sim 0$ms & $\sim 0$ms & $39.61 \pm 1.47$\\
	e-Greedy (e = 0.2, GC) & $\sim 0$ms & $\sim 0$ms & $38.62 \pm 1.42$\\
	e-Greedy (e = 0.3, GC) & $\sim 0$ms & $\sim 0$ms & $37.54 \pm 1.38$\\
	e-Greedy (e = 0.4, GC) & $\sim 0$ms & $\sim 0$ms & $36.1 \pm 1.19$\\
	e-Greedy (e = 0.5, GC) & $\sim 0$ms & $\sim 0$ms & $36.41 \pm 1.3$\\
	e-Greedy (e = 0.6, GC) & $\sim 0$ms & $\sim 0$ms & $34.44 \pm 1.08$\\
	e-Greedy (e = 0.7, GC) & $\sim 0$ms & $\sim 0$ms & $33.89 \pm 1.15$\\
	e-Greedy (e = 0.8, GC) & $\sim 0$ms & $\sim 0$ms & $32.98 \pm 1.08$\\
	e-Greedy (e = 0.9, GC) & $\sim 0$ms & $\sim 0$ms & $32.77 \pm 1.13$\\
	e-Greedy (e = 1, GC) & $\sim 0$ms & $\sim 0$ms & $31.22 \pm 0.95$\\
	Soft-Max (tau = 0.05, GC) & $\sim 0$ms & $\sim 0$ms & $33.42 \pm 1.4$\\
	\textbf{Soft-Max (tau = 0.1, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{34.73 \pm 1.74}$\\
	Soft-Max (tau = 0.2, GC) & $\sim 0$ms & $\sim 0$ms & $34.46 \pm 1.64$\\
	Soft-Max (tau = 0.33, GC) & $\sim 0$ms & $\sim 0$ms & $34.22 \pm 1.57$\\
	Soft-Max (tau = 0.5, GC) & $\sim 0$ms & $\sim 0$ms & $34.46 \pm 1.64$\\
	Soft-Max (tau = 1, GC) & $\sim 0$ms & $\sim 0$ms & $33.63 \pm 1.44$\\
	Soft-Max (tau = 2, GC) & $\sim 0$ms & $\sim 0$ms & $34.22 \pm 1.57$\\
	Soft-Max (tau = 3, GC) & $\sim 0$ms & $\sim 0$ms & $34.22 \pm 1.57$\\
	Soft-Max (tau = 5, GC) & $\sim 0$ms & $\sim 0$ms & $33.63 \pm 1.44$\\
	Soft-Max (tau = 25, GC) & $\sim 0$ms & $\sim 0$ms & $34.2 \pm 1.62$\\
	OPPS-DS (Formula (X2 INV), GC) & $\sim 641$ms & $\sim 0$ms & $30.21 \pm 1.01$\\
	OPPS-DS (Formula (X0 ABS), GC) & $\sim 11$s & $\sim 0$ms & $41.06 \pm 1.59$\\
	OPPS-DS (Formula (X0), GC) & $\sim 16$s & $\sim 0$ms & $41.47 \pm 1.72$\\
	OPPS-DS (Formula (X0), GC) & $\sim 33$s & $\sim 0$ms & $41.47 \pm 1.72$\\
	OPPS-DS (Formula (X0), GC) & $\sim 2$m & $\sim 0$ms & $41.47 \pm 1.72$\\
	OPPS-DS (Formula (X0), GC) & $\sim 2$m & $\sim 0$ms & $41.47 \pm 1.72$\\
	OPPS-DS (Formula (X0), GC) & $\sim 21$m & $\sim 0$ms & $39.97 \pm 1.55$\\
	OPPS-DS (Formula (X0 ABS), GC) & $\sim 3$h & $\sim 0$ms & $40.93 \pm 1.66$\\
	OPPS-DS (Formula (X2), GC) & $\sim 1$s & $\sim 0$ms & $37.46 \pm 1.59$\\
	OPPS-DS (Formula (X0 ABS), GC) & $\sim 10$s & $\sim 0$ms & $40.93 \pm 1.66$\\
	OPPS-DS (Formula (X1 X0 ADD2), GC) & $\sim 25$s & $\sim 0$ms & $38.63 \pm 1.59$\\
	\textbf{OPPS-DS (Formula (X0 X2 DIV), GC)} & $\boldsymbol{\sim 50}$\textbf{s} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{42.47 \pm 1.91}$\\
	OPPS-DS (Formula (X2 X0 MIN2), GC) & $\sim 2$m & $\sim 0$ms & $41.67 \pm 1.85$\\
	OPPS-DS (Formula (X2 X0 ADD2), GC) & $\sim 3$m & $\sim 0$ms & $41.05 \pm 1.74$\\
	\textbf{OPPS-DS (Formula (X0 X2 DIV), GC)} & $\boldsymbol{\sim 34}$\textbf{m} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{41.82 \pm 1.83}$\\
	OPPS-DS (Formula (X0 ABS), GC) & $\sim 6$h & $\sim 0$ms & $41.95 \pm 1.73$\\
	OPPS-DS (Formula (X2 ABS X0 MIN2), GC) & $\sim 28$s & $\sim 0$ms & $41.92 \pm 1.73$\\
	OPPS-DS (Formula (X0 INV X0 MAX2), GC) & $\sim 57$s & $\sim 0$ms & $41.06 \pm 1.59$\\
	OPPS-DS (Formula (X2 OPP X0 DIV), GC) & $\sim 2$m & $\sim 0$ms & $41.82 \pm 1.83$\\
	OPPS-DS (Formula (X2 INV X0 ADD2), GC) & $\sim 4$m & $\sim 0$ms & $41.95 \pm 1.75$\\
	OPPS-DS (Formula (X0 X2 DIV ABS), GC) & $\sim 55$m & $\sim 0$ms & $41.84 \pm 1.99$\\
	OPPS-DS (Formula (X0 X0 INV SUB), GC) & $\sim 6$h & $\sim 0$ms & $41.95 \pm 1.73$\\
	OPPS-DS (Formula (X2 X0 ABS MIN2 ABS), GC) & $\sim 32$s & $\sim 0$ms & $40.09 \pm 1.55$\\
	OPPS-DS (Formula (X2 X0 MIN2 X0 MUL2), GC) & $\sim 1$m & $\sim 0$ms & $40.26 \pm 1.59$\\
	OPPS-DS (Formula (X2 INV X0 ADD2 ABS), GC) & $\sim 2$m & $\sim 0$ms & $41.95 \pm 1.75$\\
	OPPS-DS (Formula (X2 X1 ADD2 X0 MAX2), GC) & $\sim 4$m & $\sim 0$ms & $36.87 \pm 1.64$\\
	OPPS-DS (Formula (X2 X0 ABS MIN2), GC) & $\sim 42$m & $\sim 0$ms & $41.44 \pm 1.69$\\
	OPPS-DS (Formula (X1 X0 X0 MUL2 MAX2), GC) & $\sim 7$h & $\sim 0$ms & $41.89 \pm 1.69$\\
	OPPS-DS (Formula (X0 X2 INV X2 DIV SUB), GC) & $\sim 3$m & $\sim 0$ms & $40.76 \pm 1.66$\\
	OPPS-DS (Formula (X2 X0 ABS MAX2 X0 ADD2), GC) & $\sim 5$m & $\sim 0$ms & $40.44 \pm 1.75$\\
	OPPS-DS (Formula (X2 X0 X0 ADD2 ABS ADD2), GC) & $\sim 46$m & $\sim 0$ms & $40.59 \pm 1.63$\\
	OPPS-DS (Formula (X0 X2 X0 INV SUB DIV), GC) & $\sim 8$h & $\sim 0$ms & $41.34 \pm 1.78$\\
	BAMCP (K = 1, depth = 15, GC) & $\sim 0$ms & $\sim 0$ms & $31.33 \pm 0.98$\\
	BAMCP (K = 1, depth = 25, GC) & $\sim 0$ms & $\sim 0$ms & $30.88 \pm 0.91$\\
	BAMCP (K = 1, depth = 50, GC) & $\sim 0$ms & $\sim 0$ms & $32.15 \pm 1.07$\\
	BAMCP (K = 500, depth = 15, GC) & $\sim 0$ms & $\sim 4$ms & $35.27 \pm 1.16$\\
	BAMCP (K = 500, depth = 25, GC) & $\sim 0$ms & $\sim 4$ms & $34.58 \pm 1.12$\\
	BAMCP (K = 500, depth = 50, GC) & $\sim 0$ms & $\sim 5$ms & $34.47 \pm 1.27$\\
	BAMCP (K = 1250, depth = 15, GC) & $\sim 0$ms & $\sim 10$ms & $35.52 \pm 1.15$\\
	BAMCP (K = 1250, depth = 25, GC) & $\sim 0$ms & $\sim 11$ms & $34.58 \pm 1$\\
	BAMCP (K = 1250, depth = 50, GC) & $\sim 0$ms & $\sim 12$ms & $34.47 \pm 1.05$\\
	\textbf{BAMCP (K = 2500, depth = 15, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 20}$\textbf{ms} & $\boldsymbol{35.56 \pm 1.27}$\\
	BAMCP (K = 2500, depth = 25, GC) & $\sim 0$ms & $\sim 23$ms & $34.3 \pm 1.1$\\
	BAMCP (K = 2500, depth = 50, GC) & $\sim 0$ms & $\sim 26$ms & $33.86 \pm 1.05$\\
	BAMCP (K = 5000, depth = 15, GC) & $\sim 0$ms & $\sim 38$ms & $34.81 \pm 1.08$\\
	BAMCP (K = 5000, depth = 25, GC) & $\sim 0$ms & $\sim 49$ms & $35.01 \pm 1.13$\\
	BAMCP (K = 5000, depth = 50, GC) & $\sim 0$ms & $\sim 51$ms & $34.07 \pm 1.06$\\
	BAMCP (K = 10000, depth = 15, GC) & $\sim 0$ms & $\sim 89$ms & $35.16 \pm 1.06$\\
	BAMCP (K = 10000, depth = 25, GC) & $\sim 0$ms & $\sim 92$ms & $34.94 \pm 1.05$\\
	BAMCP (K = 10000, depth = 50, GC) & $\sim 0$ms & $\sim 166$ms & $34.86 \pm 1.27$\\
	BAMCP (K = 25000, depth = 15, GC) & $\sim 0$ms & $\sim 398$ms & $34.4 \pm 0.95$\\
	BAMCP (K = 25000, depth = 25, GC) & $\sim 0$ms & $\sim 229$ms & $34.49 \pm 1.12$\\
	BAMCP (K = 25000, depth = 50, GC) & $\sim 0$ms & $\sim 265$ms & $35.51 \pm 1.22$\\
	BFS3 (K = 1, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 0$ms & $33.44 \pm 1.13$\\
	BFS3 (K = 1, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 0$ms & $33.31 \pm 1.05$\\
	BFS3 (K = 1, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 0$ms & $34.27 \pm 1.09$\\
	BFS3 (K = 1, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 0$ms & $34.03 \pm 1.03$\\
	BFS3 (K = 1, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 1$ms & $34.73 \pm 1.11$\\
	BFS3 (K = 1, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 1$ms & $34.59 \pm 1.13$\\
	BFS3 (K = 1, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 1$ms & $35.55 \pm 1.18$\\
	BFS3 (K = 1, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 2$ms & $36 \pm 1.29$\\
	BFS3 (K = 1, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 3$ms & $35.73 \pm 1.34$\\
	BFS3 (K = 1, C = 15, depth = 15, GC) & $\sim 0$ms & $\sim 2$ms & $35.15 \pm 1.26$\\
	BFS3 (K = 1, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 3$ms & $35.83 \pm 1.29$\\
	BFS3 (K = 1, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 6$ms & $36.27 \pm 1.38$\\
	BFS3 (K = 500, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 19$ms & $33.3 \pm 1.14$\\
	BFS3 (K = 500, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 37$ms & $34.1 \pm 1.27$\\
	BFS3 (K = 500, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 83$ms & $33.49 \pm 1.13$\\
	BFS3 (K = 500, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 17$ms & $34.91 \pm 1.37$\\
	BFS3 (K = 500, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 39$ms & $35.68 \pm 1.34$\\
	BFS3 (K = 500, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 111$ms & $36.93 \pm 1.54$\\
	BFS3 (K = 500, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 32$ms & $37.95 \pm 1.53$\\
	BFS3 (K = 500, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 63$ms & $37.24 \pm 1.54$\\
	BFS3 (K = 500, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 142$ms & $37.49 \pm 1.48$\\
	\textbf{BFS3 (K = 500, C = 15, depth = 15, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 45}$\textbf{ms} & $\boldsymbol{39.84 \pm 1.74}$\\
	BFS3 (K = 500, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 79$ms & $39.59 \pm 1.82$\\
	BFS3 (K = 500, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 210$ms & $39.29 \pm 1.75$\\
	BFS3 (K = 1250, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 43$ms & $33.3 \pm 1.25$\\
	BFS3 (K = 1250, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 94$ms & $33.54 \pm 1.14$\\
	BFS3 (K = 1250, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 226$ms & $33.06 \pm 1.11$\\
	BFS3 (K = 1250, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 28$ms & $35.4 \pm 1.31$\\
	BFS3 (K = 1250, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 68$ms & $35.26 \pm 1.24$\\
	BFS3 (K = 1250, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 219$ms & $36.39 \pm 1.36$\\
	BFS3 (K = 1250, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 63$ms & $37.28 \pm 1.55$\\
	BFS3 (K = 1250, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 138$ms & $37.47 \pm 1.64$\\
	BFS3 (K = 1250, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 313$ms & $36.51 \pm 1.45$\\
	BFS3 (K = 1250, C = 15, depth = 15, GC) & $\sim 0$ms & $\sim 86$ms & $38.96 \pm 1.67$\\
	BFS3 (K = 1250, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 191$ms & $38.99 \pm 1.7$\\
	BFS3 (K = 1250, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 412$ms & $38.14 \pm 1.59$\\
	BFS3 (K = 2500, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 80$ms & $34.26 \pm 1.27$\\
	BFS3 (K = 2500, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 171$ms & $32.7 \pm 1.09$\\
	BFS3 (K = 2500, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 423$ms & $33.96 \pm 1.18$\\
	BFS3 (K = 2500, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 43$ms & $35.45 \pm 1.21$\\
	BFS3 (K = 2500, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 94$ms & $35.6 \pm 1.35$\\
	BFS3 (K = 2500, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 337$ms & $35.46 \pm 1.32$\\
	BFS3 (K = 2500, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 150$ms & $37.64 \pm 1.48$\\
	BFS3 (K = 2500, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 197$ms & $38.68 \pm 1.76$\\
	BFS3 (K = 2500, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 513$ms & $37.24 \pm 1.58$\\
	BFS3 (K = 2500, C = 15, depth = 15, GC) & $\sim 0$ms & $\sim 136$ms & $38.5 \pm 1.56$\\
	BFS3 (K = 2500, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 479$ms & $39.79 \pm 1.74$\\
	BFS3 (K = 2500, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 732$ms & $37.59 \pm 1.63$\\
	BFS3 (K = 5000, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 150$ms & $33.04 \pm 1.01$\\
	BFS3 (K = 5000, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 315$ms & $33.18 \pm 1.15$\\
	BFS3 (K = 5000, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 829$ms & $33.52 \pm 1.32$\\
	BFS3 (K = 5000, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 75$ms & $35.43 \pm 1.31$\\
	BFS3 (K = 5000, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 149$ms & $35.43 \pm 1.23$\\
	BFS3 (K = 5000, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 505$ms & $35.86 \pm 1.39$\\
	BFS3 (K = 5000, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 128$ms & $37.51 \pm 1.48$\\
	BFS3 (K = 5000, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 339$ms & $37.86 \pm 1.66$\\
	BFS3 (K = 5000, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 898$ms & $37.09 \pm 1.55$\\
	BFS3 (K = 5000, C = 15, depth = 15, GC) & $\sim 0$ms & $\sim 343$ms & $37.66 \pm 1.48$\\
	BFS3 (K = 5000, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 515$ms & $38.47 \pm 1.7$\\
	BFS3 (K = 5000, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 1$s & $38.72 \pm 1.66$\\
	BFS3 (K = 10000, C = 2, depth = 15, GC) & $\sim 0$ms & $\sim 295$ms & $33.57 \pm 1.27$\\
	BFS3 (K = 10000, C = 2, depth = 25, GC) & $\sim 0$ms & $\sim 614$ms & $33.14 \pm 1.06$\\
	BFS3 (K = 10000, C = 2, depth = 50, GC) & $\sim 0$ms & $\sim 2$s & $33.3 \pm 1.14$\\
	BFS3 (K = 10000, C = 5, depth = 15, GC) & $\sim 0$ms & $\sim 133$ms & $36.33 \pm 1.37$\\
	BFS3 (K = 10000, C = 5, depth = 25, GC) & $\sim 0$ms & $\sim 241$ms & $35.65 \pm 1.27$\\
	BFS3 (K = 10000, C = 5, depth = 50, GC) & $\sim 0$ms & $\sim 705$ms & $36.01 \pm 1.28$\\
	BFS3 (K = 10000, C = 10, depth = 15, GC) & $\sim 0$ms & $\sim 192$ms & $36.85 \pm 1.41$\\
	BFS3 (K = 10000, C = 10, depth = 25, GC) & $\sim 0$ms & $\sim 413$ms & $38.53 \pm 1.59$\\
	BFS3 (K = 10000, C = 10, depth = 50, GC) & $\sim 0$ms & $\sim 1$s & $38.52 \pm 1.71$\\
	BFS3 (K = 10000, C = 15, depth = 15, GC) & $\sim 0$ms & $\sim 271$ms & $39.48 \pm 1.68$\\
	BFS3 (K = 10000, C = 15, depth = 25, GC) & $\sim 0$ms & $\sim 671$ms & $39.09 \pm 1.65$\\
	BFS3 (K = 10000, C = 15, depth = 50, GC) & $\sim 0$ms & $\sim 2$s & $38.64 \pm 1.62$\\
	SBOSS (epsilon = 1, delta = 9, GC) & $\sim 0$ms & $\sim 0$ms & $34.21 \pm 1.58$\\
	SBOSS (epsilon = 1, delta = 7, GC) & $\sim 0$ms & $\sim 0$ms & $33.35 \pm 1.51$\\
	SBOSS (epsilon = 1, delta = 5, GC) & $\sim 0$ms & $\sim 0$ms & $33.51 \pm 1.55$\\
	SBOSS (epsilon = 1, delta = 3, GC) & $\sim 0$ms & $\sim 0$ms & $33.54 \pm 1.49$\\
	SBOSS (epsilon = 1, delta = 1, GC) & $\sim 0$ms & $\sim 0$ms & $34.82 \pm 1.61$\\
	SBOSS (epsilon = 1, delta = 0.1, GC) & $\sim 0$ms & $\sim 0$ms & $33.98 \pm 1.64$\\
	SBOSS (epsilon = 1, delta = 0.01, GC) & $\sim 0$ms & $\sim 0$ms & $34.9 \pm 1.68$\\
	SBOSS (epsilon = 1, delta = 0.001, GC) & $\sim 0$ms & $\sim 0$ms & $33.28 \pm 1.42$\\
	SBOSS (epsilon = 0.1, delta = 9, GC) & $\sim 0$ms & $\sim 0$ms & $34.12 \pm 1.61$\\
	SBOSS (epsilon = 0.1, delta = 7, GC) & $\sim 0$ms & $\sim 0$ms & $33.89 \pm 1.83$\\
	SBOSS (epsilon = 0.1, delta = 5, GC) & $\sim 0$ms & $\sim 0$ms & $33.73 \pm 1.57$\\
	SBOSS (epsilon = 0.1, delta = 3, GC) & $\sim 0$ms & $\sim 0$ms & $34.76 \pm 1.73$\\
	SBOSS (epsilon = 0.1, delta = 1, GC) & $\sim 0$ms & $\sim 0$ms & $34.99 \pm 1.83$\\
	SBOSS (epsilon = 0.1, delta = 0.1, GC) & $\sim 0$ms & $\sim 0$ms & $34.45 \pm 1.69$\\
	SBOSS (epsilon = 0.1, delta = 0.01, GC) & $\sim 0$ms & $\sim 0$ms & $33.15 \pm 1.38$\\
	SBOSS (epsilon = 0.1, delta = 0.001, GC) & $\sim 0$ms & $\sim 0$ms & $34.8 \pm 1.57$\\
	SBOSS (epsilon = 0.01, delta = 9, GC) & $\sim 0$ms & $\sim 0$ms & $33.79 \pm 1.49$\\
	SBOSS (epsilon = 0.01, delta = 7, GC) & $\sim 0$ms & $\sim 0$ms & $34.54 \pm 1.66$\\
	SBOSS (epsilon = 0.01, delta = 5, GC) & $\sim 0$ms & $\sim 0$ms & $34.59 \pm 1.58$\\
	SBOSS (epsilon = 0.01, delta = 3, GC) & $\sim 0$ms & $\sim 0$ms & $34.35 \pm 1.73$\\
	SBOSS (epsilon = 0.01, delta = 1, GC) & $\sim 0$ms & $\sim 0$ms & $33.79 \pm 1.54$\\
	SBOSS (epsilon = 0.01, delta = 0.1, GC) & $\sim 0$ms & $\sim 0$ms & $33.94 \pm 1.68$\\
	SBOSS (epsilon = 0.01, delta = 0.01, GC) & $\sim 0$ms & $\sim 0$ms & $34.23 \pm 1.61$\\
	SBOSS (epsilon = 0.01, delta = 0.001, GC) & $\sim 0$ms & $\sim 0$ms & $34.7 \pm 1.68$\\
	SBOSS (epsilon = 0.001, delta = 9, GC) & $\sim 0$ms & $\sim 0$ms & $33.37 \pm 1.48$\\
	\textbf{SBOSS (epsilon = 0.001, delta = 7, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{35.9 \pm 1.89}$\\
	SBOSS (epsilon = 0.001, delta = 5, GC) & $\sim 0$ms & $\sim 0$ms & $34.24 \pm 1.78$\\
	SBOSS (epsilon = 0.001, delta = 3, GC) & $\sim 0$ms & $\sim 0$ms & $35.05 \pm 1.73$\\
	SBOSS (epsilon = 0.001, delta = 1, GC) & $\sim 0$ms & $\sim 0$ms & $35.2 \pm 1.8$\\
	SBOSS (epsilon = 0.001, delta = 0.1, GC) & $\sim 0$ms & $\sim 0$ms & $33.78 \pm 1.54$\\
	SBOSS (epsilon = 0.001, delta = 0.01, GC) & $\sim 0$ms & $\sim 0$ms & $35.57 \pm 1.77$\\
	SBOSS (epsilon = 0.001, delta = 0.001, GC) & $\sim 0$ms & $\sim 0$ms & $33.74 \pm 1.46$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, GC) & $\sim 0$ms & $\sim 0$ms & $34.09 \pm 1.66$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, GC) & $\sim 0$ms & $\sim 0$ms & $34.08 \pm 1.51$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, GC) & $\sim 0$ms & $\sim 0$ms & $33.81 \pm 1.57$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, GC) & $\sim 0$ms & $\sim 3$ms & $34.09 \pm 1.62$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, GC) & $\sim 0$ms & $\sim 3$ms & $32.12 \pm 1.35$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, GC) & $\sim 0$ms & $\sim 3$ms & $34.94 \pm 1.81$\\
	SBOSS (epsilon = 1e-06, delta = 0.0001, GC) & $\sim 0$ms & $\sim 36$ms & $32.9 \pm 1.41$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, GC) & $\sim 0$ms & $\sim 66$ms & $34.18 \pm 1.7$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, GC) & $\sim 0$ms & $\sim 43$ms & $33.67 \pm 1.59$\\
	BEB (beta = 0.25, GC) & $\sim 0$ms & $\sim 0$ms & $40.62 \pm 1.6$\\
	BEB (beta = 0.5, GC) & $\sim 0$ms & $\sim 0$ms & $40.62 \pm 1.6$\\
	BEB (beta = 1, GC) & $\sim 0$ms & $\sim 0$ms & $41.27 \pm 1.67$\\
	BEB (beta = 1.5, GC) & $\sim 0$ms & $\sim 0$ms & $40.6 \pm 1.57$\\
	BEB (beta = 2, GC) & $\sim 0$ms & $\sim 0$ms & $41.45 \pm 1.7$\\
	\textbf{BEB (beta = 2.5, GC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{41.72 \pm 1.63}$\\
	BEB (beta = 3, GC) & $\sim 0$ms & $\sim 0$ms & $41.25 \pm 1.65$\\
	BEB (beta = 4, GC) & $\sim 0$ms & $\sim 0$ms & $40.8 \pm 1.65$\\
	BEB (beta = 8, GC) & $\sim 0$ms & $\sim 0$ms & $39.93 \pm 1.61$\\
	BEB (beta = 16, GC) & $\sim 0$ms & $\sim 0$ms & $39.83 \pm 1.64$\\
\end{longtable}


==> data/table-accurate-1.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.79 \pm 0.07}$\\
	e-Greedy (e = 0, GDL) & $\sim 0$ms & $\sim 0$ms & $3.04 \pm 0.07$\\
	\textbf{e-Greedy (e = 0.1, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{3.05 \pm 0.07}$\\
	e-Greedy (e = 0.2, GDL) & $\sim 0$ms & $\sim 0$ms & $3.03 \pm 0.07$\\
	e-Greedy (e = 0.3, GDL) & $\sim 0$ms & $\sim 0$ms & $3.01 \pm 0.07$\\
	e-Greedy (e = 0.4, GDL) & $\sim 0$ms & $\sim 0$ms & $2.95 \pm 0.07$\\
	e-Greedy (e = 0.5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.92 \pm 0.07$\\
	e-Greedy (e = 0.6, GDL) & $\sim 0$ms & $\sim 0$ms & $2.88 \pm 0.07$\\
	e-Greedy (e = 0.7, GDL) & $\sim 0$ms & $\sim 0$ms & $2.83 \pm 0.07$\\
	e-Greedy (e = 0.8, GDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.07$\\
	e-Greedy (e = 0.9, GDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.07$\\
	e-Greedy (e = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	Soft-Max (tau = 0.05, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	\textbf{Soft-Max (tau = 0.1, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.79 \pm 0.1}$\\
	Soft-Max (tau = 0.2, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	Soft-Max (tau = 0.33, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	Soft-Max (tau = 0.5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	Soft-Max (tau = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	Soft-Max (tau = 2, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	Soft-Max (tau = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	Soft-Max (tau = 5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.1$\\
	Soft-Max (tau = 25, GDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.1$\\
	OPPS-DS (Formula (X2 INV), GDL) & $\sim 629$ms & $\sim 0$ms & $2.69 \pm 0.09$\\
	OPPS-DS (Formula (X0 ABS), GDL) & $\sim 8$s & $\sim 0$ms & $3.07 \pm 0.07$\\
	OPPS-DS (Formula (X2 OPP), GDL) & $\sim 19$s & $\sim 0$ms & $2.68 \pm 0.09$\\
	OPPS-DS (Formula (X2 ABS), GDL) & $\sim 38$s & $\sim 0$ms & $2.87 \pm 0.08$\\
	OPPS-DS (Formula (X0 ABS), GDL) & $\sim 1$m & $\sim 0$ms & $3.05 \pm 0.07$\\
	OPPS-DS (Formula (X0), GDL) & $\sim 3$m & $\sim 0$ms & $3.01 \pm 0.07$\\
	OPPS-DS (Formula (X0), GDL) & $\sim 26$m & $\sim 0$ms & $3.06 \pm 0.07$\\
	OPPS-DS (Formula (X0), GDL) & $\sim 4$h & $\sim 0$ms & $3.06 \pm 0.07$\\
	OPPS-DS (Formula (X1 X0 SUB), GDL) & $\sim 1$s & $\sim 0$ms & $2.63 \pm 0.1$\\
	OPPS-DS (Formula (X2 X1 SUB), GDL) & $\sim 12$s & $\sim 0$ms & $2.65 \pm 0.08$\\
	OPPS-DS (Formula (X2 X1 MUL2), GDL) & $\sim 18$s & $\sim 0$ms & $2.85 \pm 0.08$\\
	OPPS-DS (Formula (X0 ABS), GDL) & $\sim 35$s & $\sim 0$ms & $3.04 \pm 0.08$\\
	OPPS-DS (Formula (X1 ABS), GDL) & $\sim 2$m & $\sim 0$ms & $2.87 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 ADD2), GDL) & $\sim 4$m & $\sim 0$ms & $3.05 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 ADD2), GDL) & $\sim 41$m & $\sim 0$ms & $3.01 \pm 0.07$\\
	OPPS-DS (Formula (X2 X0 ADD2), GDL) & $\sim 7$h & $\sim 0$ms & $3.01 \pm 0.07$\\
	OPPS-DS (Formula (X2 X0 MUL2), GDL) & $\sim 19$s & $\sim 0$ms & $3.09 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 ADD2), GDL) & $\sim 1$m & $\sim 0$ms & $3.01 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 ADD2 ABS), GDL) & $\sim 2$m & $\sim 0$ms & $3.09 \pm 0.07$\\
	OPPS-DS (Formula (X2 X0 MUL2), GDL) & $\sim 5$m & $\sim 0$ms & $3 \pm 0.07$\\
	OPPS-DS (Formula (X2 X0 MAX2), GDL) & $\sim 46$m & $\sim 0$ms & $3.02 \pm 0.07$\\
	\textbf{OPPS-DS (Formula (X2 ABS X0 MAX2), GDL)} & $\boldsymbol{\sim 4}$\textbf{h} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{3.1 \pm 0.07}$\\
	OPPS-DS (Formula (X2 X2 X0 MAX2 MUL2), GDL) & $\sim 22$s & $\sim 0$ms & $3.05 \pm 0.07$\\
	OPPS-DS (Formula (X2 X0 ABS OPP MAX2), GDL) & $\sim 43$s & $\sim 0$ms & $2.89 \pm 0.07$\\
	OPPS-DS (Formula (X2 X2 X1 ADD2 MUL2), GDL) & $\sim 1$m & $\sim 0$ms & $2.97 \pm 0.07$\\
	OPPS-DS (Formula (X0 X2 X0 ADD2 DIV), GDL) & $\sim 5$m & $\sim 0$ms & $3.03 \pm 0.07$\\
	OPPS-DS (Formula (X2 X1 X0 MAX2 MUL2), GDL) & $\sim 52$m & $\sim 0$ms & $3.05 \pm 0.07$\\
	OPPS-DS (Formula (X0 X0 INV ABS SUB), GDL) & $\sim 5$h & $\sim 0$ms & $3.04 \pm 0.07$\\
	OPPS-DS (Formula (X2 X1 ABS SQRT SQRT ADD2), GDL) & $\sim 4$m & $\sim 0$ms & $2.94 \pm 0.07$\\
	OPPS-DS (Formula (X0 ABS LN X0 MIN2 OPP), GDL) & $\sim 6$m & $\sim 0$ms & $2.31 \pm 0.09$\\
	OPPS-DS (Formula (X2 ABS SQRT SQRT X1 SUB), GDL) & $\sim 55$m & $\sim 0$ms & $2.61 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 ABS X0 DIV MAX2), GDL) & $\sim 9$h & $\sim 0$ms & $2.92 \pm 0.07$\\
	BAMCP (K = 1, depth = 15, GDL) & $\sim 0$ms & $\sim 0$ms & $2.74 \pm 0.07$\\
	BAMCP (K = 1, depth = 25, GDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.08$\\
	BAMCP (K = 1, depth = 50, GDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.07$\\
	BAMCP (K = 500, depth = 15, GDL) & $\sim 0$ms & $\sim 8$ms & $3.05 \pm 0.08$\\
	BAMCP (K = 500, depth = 25, GDL) & $\sim 0$ms & $\sim 8$ms & $3.05 \pm 0.07$\\
	BAMCP (K = 500, depth = 50, GDL) & $\sim 0$ms & $\sim 9$ms & $3 \pm 0.07$\\
	BAMCP (K = 1250, depth = 15, GDL) & $\sim 0$ms & $\sim 20$ms & $3.04 \pm 0.07$\\
	BAMCP (K = 1250, depth = 25, GDL) & $\sim 0$ms & $\sim 21$ms & $3.02 \pm 0.07$\\
	BAMCP (K = 1250, depth = 50, GDL) & $\sim 0$ms & $\sim 23$ms & $3.06 \pm 0.07$\\
	BAMCP (K = 2500, depth = 15, GDL) & $\sim 0$ms & $\sim 42$ms & $3.07 \pm 0.08$\\
	BAMCP (K = 2500, depth = 25, GDL) & $\sim 0$ms & $\sim 41$ms & $3.07 \pm 0.07$\\
	BAMCP (K = 2500, depth = 50, GDL) & $\sim 0$ms & $\sim 45$ms & $3.07 \pm 0.07$\\
	BAMCP (K = 5000, depth = 15, GDL) & $\sim 0$ms & $\sim 83$ms & $3.01 \pm 0.07$\\
	BAMCP (K = 5000, depth = 25, GDL) & $\sim 0$ms & $\sim 148$ms & $3.02 \pm 0.07$\\
	BAMCP (K = 5000, depth = 50, GDL) & $\sim 0$ms & $\sim 101$ms & $3.04 \pm 0.08$\\
	\textbf{BAMCP (K = 10000, depth = 15, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 263}$\textbf{ms} & $\boldsymbol{3.11 \pm 0.07}$\\
	BAMCP (K = 10000, depth = 25, GDL) & $\sim 0$ms & $\sim 172$ms & $3.04 \pm 0.07$\\
	BAMCP (K = 10000, depth = 50, GDL) & $\sim 0$ms & $\sim 188$ms & $3 \pm 0.07$\\
	BAMCP (K = 25000, depth = 15, GDL) & $\sim 0$ms & $\sim 427$ms & $3.05 \pm 0.07$\\
	BAMCP (K = 25000, depth = 25, GDL) & $\sim 0$ms & $\sim 732$ms & $3.09 \pm 0.07$\\
	BAMCP (K = 25000, depth = 50, GDL) & $\sim 0$ms & $\sim 479$ms & $3.1 \pm 0.07$\\
	BFS3 (K = 1, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 1, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.08$\\
	BFS3 (K = 1, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 0$ms & $2.84 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 0$ms & $2.86 \pm 0.08$\\
	BFS3 (K = 1, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 1$ms & $2.82 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 1$ms & $2.84 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 1$ms & $2.77 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 2$ms & $2.79 \pm 0.08$\\
	BFS3 (K = 1, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 1$ms & $2.8 \pm 0.07$\\
	\textbf{BFS3 (K = 1, C = 15, depth = 25, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{2.9 \pm 0.07}$\\
	BFS3 (K = 1, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 3$ms & $2.87 \pm 0.07$\\
	BFS3 (K = 500, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 11$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 500, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 21$ms & $2.73 \pm 0.08$\\
	BFS3 (K = 500, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 49$ms & $2.74 \pm 0.08$\\
	BFS3 (K = 500, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 12$ms & $2.65 \pm 0.08$\\
	BFS3 (K = 500, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 25$ms & $2.62 \pm 0.09$\\
	BFS3 (K = 500, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 60$ms & $2.58 \pm 0.08$\\
	BFS3 (K = 500, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 16$ms & $2.72 \pm 0.09$\\
	BFS3 (K = 500, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 31$ms & $2.74 \pm 0.09$\\
	BFS3 (K = 500, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 69$ms & $2.68 \pm 0.09$\\
	BFS3 (K = 500, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 22$ms & $2.69 \pm 0.09$\\
	BFS3 (K = 500, C = 15, depth = 25, GDL) & $\sim 0$ms & $\sim 38$ms & $2.67 \pm 0.09$\\
	BFS3 (K = 500, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 83$ms & $2.71 \pm 0.09$\\
	BFS3 (K = 1250, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 25$ms & $2.74 \pm 0.08$\\
	BFS3 (K = 1250, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 51$ms & $2.77 \pm 0.08$\\
	BFS3 (K = 1250, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 119$ms & $2.71 \pm 0.08$\\
	BFS3 (K = 1250, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 20$ms & $2.65 \pm 0.08$\\
	BFS3 (K = 1250, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 47$ms & $2.7 \pm 0.09$\\
	BFS3 (K = 1250, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 125$ms & $2.68 \pm 0.08$\\
	BFS3 (K = 1250, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 34$ms & $2.66 \pm 0.09$\\
	BFS3 (K = 1250, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 72$ms & $2.72 \pm 0.09$\\
	BFS3 (K = 1250, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 188$ms & $2.66 \pm 0.09$\\
	BFS3 (K = 1250, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 46$ms & $2.67 \pm 0.09$\\
	BFS3 (K = 1250, C = 15, depth = 25, GDL) & $\sim 0$ms & $\sim 97$ms & $2.72 \pm 0.08$\\
	BFS3 (K = 1250, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 206$ms & $2.68 \pm 0.09$\\
	BFS3 (K = 2500, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 81$ms & $2.76 \pm 0.08$\\
	BFS3 (K = 2500, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 100$ms & $2.72 \pm 0.08$\\
	BFS3 (K = 2500, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 232$ms & $2.68 \pm 0.08$\\
	BFS3 (K = 2500, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 29$ms & $2.64 \pm 0.08$\\
	BFS3 (K = 2500, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 65$ms & $2.66 \pm 0.09$\\
	BFS3 (K = 2500, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 196$ms & $2.64 \pm 0.08$\\
	BFS3 (K = 2500, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 52$ms & $2.64 \pm 0.08$\\
	BFS3 (K = 2500, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 126$ms & $2.62 \pm 0.09$\\
	BFS3 (K = 2500, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 502$ms & $2.61 \pm 0.09$\\
	BFS3 (K = 2500, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 71$ms & $2.69 \pm 0.09$\\
	BFS3 (K = 2500, C = 15, depth = 25, GDL) & $\sim 0$ms & $\sim 168$ms & $2.65 \pm 0.09$\\
	BFS3 (K = 2500, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 405$ms & $2.73 \pm 0.09$\\
	BFS3 (K = 5000, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 82$ms & $2.75 \pm 0.08$\\
	BFS3 (K = 5000, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 193$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 5000, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 438$ms & $2.69 \pm 0.08$\\
	BFS3 (K = 5000, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 44$ms & $2.66 \pm 0.08$\\
	BFS3 (K = 5000, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 97$ms & $2.7 \pm 0.08$\\
	BFS3 (K = 5000, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 285$ms & $2.72 \pm 0.08$\\
	BFS3 (K = 5000, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 77$ms & $2.71 \pm 0.09$\\
	BFS3 (K = 5000, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 187$ms & $2.7 \pm 0.08$\\
	BFS3 (K = 5000, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 586$ms & $2.6 \pm 0.08$\\
	BFS3 (K = 5000, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 103$ms & $2.68 \pm 0.09$\\
	BFS3 (K = 5000, C = 15, depth = 25, GDL) & $\sim 0$ms & $\sim 268$ms & $2.65 \pm 0.09$\\
	BFS3 (K = 5000, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 1$s & $2.73 \pm 0.09$\\
	BFS3 (K = 10000, C = 2, depth = 15, GDL) & $\sim 0$ms & $\sim 166$ms & $2.77 \pm 0.08$\\
	BFS3 (K = 10000, C = 2, depth = 25, GDL) & $\sim 0$ms & $\sim 373$ms & $2.75 \pm 0.08$\\
	BFS3 (K = 10000, C = 2, depth = 50, GDL) & $\sim 0$ms & $\sim 906$ms & $2.73 \pm 0.08$\\
	BFS3 (K = 10000, C = 5, depth = 15, GDL) & $\sim 0$ms & $\sim 81$ms & $2.69 \pm 0.08$\\
	BFS3 (K = 10000, C = 5, depth = 25, GDL) & $\sim 0$ms & $\sim 158$ms & $2.73 \pm 0.08$\\
	BFS3 (K = 10000, C = 5, depth = 50, GDL) & $\sim 0$ms & $\sim 420$ms & $2.69 \pm 0.09$\\
	BFS3 (K = 10000, C = 10, depth = 15, GDL) & $\sim 0$ms & $\sim 113$ms & $2.69 \pm 0.08$\\
	BFS3 (K = 10000, C = 10, depth = 25, GDL) & $\sim 0$ms & $\sim 465$ms & $2.69 \pm 0.08$\\
	BFS3 (K = 10000, C = 10, depth = 50, GDL) & $\sim 0$ms & $\sim 862$ms & $2.69 \pm 0.08$\\
	BFS3 (K = 10000, C = 15, depth = 15, GDL) & $\sim 0$ms & $\sim 247$ms & $2.66 \pm 0.09$\\
	BFS3 (K = 10000, C = 15, depth = 25, GDL) & $\sim 0$ms & $\sim 392$ms & $2.65 \pm 0.08$\\
	BFS3 (K = 10000, C = 15, depth = 50, GDL) & $\sim 0$ms & $\sim 1$s & $2.72 \pm 0.08$\\
	SBOSS (epsilon = 1, delta = 9, GDL) & $\sim 0$ms & $\sim 0$ms & $2.7 \pm 0.1$\\
	SBOSS (epsilon = 1, delta = 7, GDL) & $\sim 0$ms & $\sim 0$ms & $2.7 \pm 0.1$\\
	SBOSS (epsilon = 1, delta = 5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.1$\\
	SBOSS (epsilon = 1, delta = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.1$\\
	\textbf{SBOSS (epsilon = 1, delta = 1, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.81 \pm 0.1}$\\
	SBOSS (epsilon = 1, delta = 0.1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.09$\\
	SBOSS (epsilon = 1, delta = 0.01, GDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.1$\\
	SBOSS (epsilon = 1, delta = 0.001, GDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 9, GDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.09$\\
	SBOSS (epsilon = 0.1, delta = 7, GDL) & $\sim 0$ms & $\sim 0$ms & $2.68 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.64 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 0.1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 0.01, GDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.1$\\
	SBOSS (epsilon = 0.1, delta = 0.001, GDL) & $\sim 0$ms & $\sim 0$ms & $2.65 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 9, GDL) & $\sim 0$ms & $\sim 0$ms & $2.66 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 7, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.65 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 0.1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 0.01, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.01, delta = 0.001, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 9, GDL) & $\sim 0$ms & $\sim 0$ms & $2.74 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 7, GDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.68 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.66 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 0.1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.63 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 0.01, GDL) & $\sim 0$ms & $\sim 0$ms & $2.68 \pm 0.1$\\
	SBOSS (epsilon = 0.001, delta = 0.001, GDL) & $\sim 0$ms & $\sim 0$ms & $2.65 \pm 0.1$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, GDL) & $\sim 0$ms & $\sim 1$ms & $2.71 \pm 0.09$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, GDL) & $\sim 0$ms & $\sim 1$ms & $2.71 \pm 0.09$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, GDL) & $\sim 0$ms & $\sim 1$ms & $2.68 \pm 0.1$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, GDL) & $\sim 0$ms & $\sim 7$ms & $2.69 \pm 0.1$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, GDL) & $\sim 0$ms & $\sim 8$ms & $2.77 \pm 0.09$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, GDL) & $\sim 0$ms & $\sim 8$ms & $2.73 \pm 0.1$\\
	SBOSS (epsilon = 1e-06, delta = 0.0001, GDL) & $\sim 0$ms & $\sim 73$ms & $2.7 \pm 0.1$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, GDL) & $\sim 0$ms & $\sim 76$ms & $2.66 \pm 0.1$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, GDL) & $\sim 0$ms & $\sim 75$ms & $2.69 \pm 0.1$\\
	BEB (beta = 0.25, GDL) & $\sim 0$ms & $\sim 0$ms & $3.03 \pm 0.07$\\
	\textbf{BEB (beta = 0.5, GDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{3.09 \pm 0.07}$\\
	BEB (beta = 1, GDL) & $\sim 0$ms & $\sim 0$ms & $2.99 \pm 0.08$\\
	BEB (beta = 1.5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.99 \pm 0.08$\\
	BEB (beta = 2, GDL) & $\sim 0$ms & $\sim 0$ms & $2.95 \pm 0.07$\\
	BEB (beta = 2.5, GDL) & $\sim 0$ms & $\sim 0$ms & $2.92 \pm 0.07$\\
	BEB (beta = 3, GDL) & $\sim 0$ms & $\sim 0$ms & $2.94 \pm 0.07$\\
	BEB (beta = 4, GDL) & $\sim 0$ms & $\sim 0$ms & $2.9 \pm 0.07$\\
	BEB (beta = 8, GDL) & $\sim 0$ms & $\sim 0$ms & $2.86 \pm 0.07$\\
	BEB (beta = 16, GDL) & $\sim 0$ms & $\sim 0$ms & $2.88 \pm 0.07$\\
\end{longtable}


==> data/table-accurate-2.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{0.22 \pm 0.06}$\\
	\textbf{e-Greedy (e = 0, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{6.9 \pm 0.31}$\\
	e-Greedy (e = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $5.88 \pm 0.27$\\
	e-Greedy (e = 0.2, Grid) & $\sim 0$ms & $\sim 0$ms & $4.79 \pm 0.26$\\
	e-Greedy (e = 0.3, Grid) & $\sim 0$ms & $\sim 0$ms & $4.23 \pm 0.24$\\
	e-Greedy (e = 0.4, Grid) & $\sim 0$ms & $\sim 0$ms & $3.35 \pm 0.22$\\
	e-Greedy (e = 0.5, Grid) & $\sim 0$ms & $\sim 0$ms & $2.61 \pm 0.2$\\
	e-Greedy (e = 0.6, Grid) & $\sim 0$ms & $\sim 0$ms & $1.77 \pm 0.16$\\
	e-Greedy (e = 0.7, Grid) & $\sim 0$ms & $\sim 0$ms & $1.33 \pm 0.14$\\
	e-Greedy (e = 0.8, Grid) & $\sim 0$ms & $\sim 0$ms & $0.75 \pm 0.1$\\
	e-Greedy (e = 0.9, Grid) & $\sim 0$ms & $\sim 0$ms & $0.52 \pm 0.09$\\
	e-Greedy (e = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $0.2 \pm 0.05$\\
	\textbf{Soft-Max (tau = 0.05, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{0 \pm 0}$\\
	Soft-Max (tau = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.2, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.33, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.5, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 2, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 3, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 5, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	Soft-Max (tau = 25, Grid) & $\sim 0$ms & $\sim 0$ms & $0 \pm 0$\\
	OPPS-DS (Formula (X1 OPP), Grid) & $\sim 4$s & $\sim 0$ms & $0.17 \pm 0.05$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 40$s & $\sim 0$ms & $6.47 \pm 0.3$\\
	OPPS-DS (Formula (X0 ABS), Grid) & $\sim 2$m & $\sim 0$ms & $6.74 \pm 0.3$\\
	OPPS-DS (Formula (X0 ABS), Grid) & $\sim 3$m & $\sim 0$ms & $6.79 \pm 0.3$\\
	OPPS-DS (Formula (X0 ABS), Grid) & $\sim 7$m & $\sim 0$ms & $6.79 \pm 0.3$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 13$m & $\sim 0$ms & $6.79 \pm 0.3$\\
	OPPS-DS (Formula (X0 ABS), Grid) & $\sim 2$h & $\sim 0$ms & $6.8 \pm 0.31$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 18$h & $\sim 0$ms & $6.71 \pm 0.31$\\
	OPPS-DS (Formula (X1 X0 MAX2), Grid) & $\sim 8$s & $\sim 0$ms & $6.76 \pm 0.31$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 1$m & $\sim 0$ms & $6.68 \pm 0.31$\\
	OPPS-DS (Formula (X2 X0 MUL2), Grid) & $\sim 3$m & $\sim 1$ms & $6.82 \pm 0.31$\\
	OPPS-DS (Formula (X0 ABS), Grid) & $\sim 6$m & $\sim 0$ms & $6.76 \pm 0.3$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 13$m & $\sim 0$ms & $6.81 \pm 0.31$\\
	\textbf{OPPS-DS (Formula (X2 X0 ADD2), Grid)} & $\boldsymbol{\sim 25}$\textbf{m} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{6.92 \pm 0.31}$\\
	OPPS-DS (Formula (X2 X0 MAX2), Grid) & $\sim 4$h & $\sim 1$ms & $6.89 \pm 0.3$\\
	OPPS-DS (Formula (X0), Grid) & $\sim 2$d & $\sim 0$ms & $6.47 \pm 0.3$\\
	OPPS-DS (Formula (X0 ABS X2 SUB), Grid) & $\sim 3$m & $\sim 1$ms & $6.2 \pm 0.28$\\
	\textbf{OPPS-DS (Formula (X2 X0 ADD2), Grid)} & $\boldsymbol{\sim 7}$\textbf{m} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{6.5 \pm 0.3}$\\
	\textbf{OPPS-DS (Formula (X2 X0 ADD2), Grid)} & $\boldsymbol{\sim 13}$\textbf{m} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{7.03 \pm 0.3}$\\
	OPPS-DS (Formula (X0 X2 ABS SUB), Grid) & $\sim 26$m & $\sim 1$ms & $6.18 \pm 0.28$\\
	OPPS-DS (Formula (X2 ABS X0 MAX2), Grid) & $\sim 4$h & $\sim 1$ms & $6.74 \pm 0.3$\\
	OPPS-DS (Formula (X2 OPP X0 MAX2), Grid) & $\sim 2$d & $\sim 1$ms & $6.74 \pm 0.3$\\
	OPPS-DS (Formula (X1 ABS X0 INV SUB), Grid) & $\sim 4$m & $\sim 0$ms & $6.55 \pm 0.31$\\
	OPPS-DS (Formula (X2 X0 ABS OPP MAX2), Grid) & $\sim 8$m & $\sim 1$ms & $0.65 \pm 0.1$\\
	OPPS-DS (Formula (X1 X0 MAX2 X2 SUB), Grid) & $\sim 16$m & $\sim 1$ms & $6.18 \pm 0.27$\\
	\textbf{OPPS-DS (Formula (X2 X0 ADD2), Grid)} & $\boldsymbol{\sim 31}$\textbf{m} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{7.03 \pm 0.3}$\\
	OPPS-DS (Formula (X2 OPP X0 SUB INV), Grid) & $\sim 5$h & $\sim 1$ms & $6.85 \pm 0.3$\\
	OPPS-DS (Formula (X2 X0 ADD2 X0 MAX2), Grid) & $\sim 2$d & $\sim 1$ms & $6.85 \pm 0.3$\\
	OPPS-DS (Formula (X2 ABS X1 X0 ADD2 MUL2), Grid) & $\sim 26$m & $\sim 2$ms & $6.45 \pm 0.3$\\
	OPPS-DS (Formula (X2 ABS SQRT X0 ABS ADD2), Grid) & $\sim 34$m & $\sim 1$ms & $6.49 \pm 0.3$\\
	OPPS-DS (Formula (X2 ABS LN X2 DIV), Grid) & $\sim 5$h & $\sim 1$ms & $0.57 \pm 0.09$\\
	OPPS-DS (Formula (X0 X2 INV X2 MIN2 SUB), Grid) & $\sim 2$d & $\sim 1$ms & $6.76 \pm 0.31$\\
	BAMCP (K = 1, depth = 15, Grid) & $\sim 0$ms & $\sim 0$ms & $0.31 \pm 0.07$\\
	BAMCP (K = 1, depth = 25, Grid) & $\sim 0$ms & $\sim 0$ms & $0.28 \pm 0.06$\\
	BAMCP (K = 1, depth = 50, Grid) & $\sim 0$ms & $\sim 0$ms & $0.26 \pm 0.06$\\
	BAMCP (K = 500, depth = 15, Grid) & $\sim 0$ms & $\sim 110$ms & $4.2 \pm 0.23$\\
	BAMCP (K = 500, depth = 25, Grid) & $\sim 0$ms & $\sim 117$ms & $4.6 \pm 0.24$\\
	BAMCP (K = 500, depth = 50, Grid) & $\sim 0$ms & $\sim 112$ms & $4.63 \pm 0.25$\\
	BAMCP (K = 1250, depth = 15, Grid) & $\sim 0$ms & $\sim 282$ms & $5.1 \pm 0.27$\\
	BAMCP (K = 1250, depth = 25, Grid) & $\sim 0$ms & $\sim 278$ms & $5.5 \pm 0.28$\\
	BAMCP (K = 1250, depth = 50, Grid) & $\sim 0$ms & $\sim 282$ms & $5.37 \pm 0.27$\\
	BAMCP (K = 2500, depth = 15, Grid) & $\sim 0$ms & $\sim 557$ms & $5.41 \pm 0.28$\\
	BAMCP (K = 2500, depth = 25, Grid) & $\sim 0$ms & $\sim 561$ms & $5.87 \pm 0.27$\\
	BAMCP (K = 2500, depth = 50, Grid) & $\sim 0$ms & $\sim 570$ms & $5.76 \pm 0.27$\\
	BAMCP (K = 5000, depth = 15, Grid) & $\sim 0$ms & $\sim 1$s & $5.95 \pm 0.28$\\
	BAMCP (K = 5000, depth = 25, Grid) & $\sim 0$ms & $\sim 1$s & $6.03 \pm 0.29$\\
	BAMCP (K = 5000, depth = 50, Grid) & $\sim 0$ms & $\sim 1$s & $6.14 \pm 0.27$\\
	BAMCP (K = 10000, depth = 15, Grid) & $\sim 0$ms & $\sim 2$s & $6.18 \pm 0.28$\\
	BAMCP (K = 10000, depth = 25, Grid) & $\sim 0$ms & $\sim 2$s & $6.29 \pm 0.28$\\
	BAMCP (K = 10000, depth = 50, Grid) & $\sim 0$ms & $\sim 2$s & $5.98 \pm 0.29$\\
	\textbf{BAMCP (K = 25000, depth = 15, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 7}$\textbf{s} & $\boldsymbol{6.43 \pm 0.3}$\\
	BAMCP (K = 25000, depth = 25, Grid) & $\sim 0$ms & $\sim 6$s & $6.05 \pm 0.28$\\
	BAMCP (K = 25000, depth = 50, Grid) & $\sim 0$ms & $\sim 6$s & $6.04 \pm 0.29$\\
	BFS3 (K = 1, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 0$ms & $0.62 \pm 0.1$\\
	BFS3 (K = 1, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 1$ms & $0.64 \pm 0.09$\\
	BFS3 (K = 1, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 1$ms & $0.67 \pm 0.1$\\
	BFS3 (K = 1, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 1$ms & $0.65 \pm 0.09$\\
	BFS3 (K = 1, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 2$ms & $0.69 \pm 0.09$\\
	BFS3 (K = 1, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 3$ms & $0.67 \pm 0.1$\\
	BFS3 (K = 1, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 3$ms & $0.76 \pm 0.1$\\
	BFS3 (K = 1, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 4$ms & $0.82 \pm 0.11$\\
	BFS3 (K = 1, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 8$ms & $0.68 \pm 0.1$\\
	BFS3 (K = 1, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 4$ms & $0.75 \pm 0.11$\\
	BFS3 (K = 1, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 7$ms & $0.78 \pm 0.1$\\
	BFS3 (K = 1, C = 15, depth = 50, Grid) & $\sim 0$ms & $\sim 14$ms & $0.89 \pm 0.12$\\
	BFS3 (K = 500, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 58$ms & $1.78 \pm 0.16$\\
	BFS3 (K = 500, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 114$ms & $1.81 \pm 0.16$\\
	BFS3 (K = 500, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 254$ms & $1.81 \pm 0.16$\\
	BFS3 (K = 500, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 75$ms & $2.58 \pm 0.2$\\
	BFS3 (K = 500, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 139$ms & $2.53 \pm 0.19$\\
	BFS3 (K = 500, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 296$ms & $2.48 \pm 0.19$\\
	BFS3 (K = 500, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 101$ms & $2.51 \pm 0.2$\\
	BFS3 (K = 500, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 171$ms & $2.64 \pm 0.21$\\
	BFS3 (K = 500, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 382$ms & $2.7 \pm 0.2$\\
	BFS3 (K = 500, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 124$ms & $3.32 \pm 0.24$\\
	BFS3 (K = 500, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 217$ms & $3.42 \pm 0.23$\\
	\textbf{BFS3 (K = 500, C = 15, depth = 50, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 428}$\textbf{ms} & $\boldsymbol{3.46 \pm 0.23}$\\
	BFS3 (K = 1250, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 150$ms & $1.41 \pm 0.15$\\
	BFS3 (K = 1250, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 264$ms & $1.42 \pm 0.15$\\
	BFS3 (K = 1250, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 552$ms & $1.54 \pm 0.15$\\
	BFS3 (K = 1250, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 169$ms & $2.63 \pm 0.19$\\
	BFS3 (K = 1250, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 348$ms & $2.91 \pm 0.2$\\
	BFS3 (K = 1250, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 807$ms & $2.85 \pm 0.2$\\
	BFS3 (K = 1250, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 221$ms & $2.52 \pm 0.2$\\
	BFS3 (K = 1250, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 473$ms & $2.61 \pm 0.21$\\
	BFS3 (K = 1250, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 946$ms & $2.56 \pm 0.19$\\
	BFS3 (K = 1250, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 269$ms & $3.2 \pm 0.23$\\
	BFS3 (K = 1250, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 542$ms & $3.32 \pm 0.22$\\
	BFS3 (K = 1250, C = 15, depth = 50, Grid) & $\sim 0$ms & $\sim 1$s & $3.33 \pm 0.22$\\
	BFS3 (K = 2500, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 298$ms & $2.39 \pm 0.18$\\
	BFS3 (K = 2500, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 537$ms & $2.21 \pm 0.17$\\
	BFS3 (K = 2500, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 1$s & $2.27 \pm 0.17$\\
	BFS3 (K = 2500, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 302$ms & $3.06 \pm 0.22$\\
	BFS3 (K = 2500, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 539$ms & $2.88 \pm 0.2$\\
	BFS3 (K = 2500, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 1$s & $2.93 \pm 0.21$\\
	BFS3 (K = 2500, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 411$ms & $2.5 \pm 0.2$\\
	BFS3 (K = 2500, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 842$ms & $2.64 \pm 0.2$\\
	BFS3 (K = 2500, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 2$s & $2.44 \pm 0.19$\\
	BFS3 (K = 2500, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 499$ms & $2.94 \pm 0.21$\\
	BFS3 (K = 2500, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 956$ms & $2.74 \pm 0.19$\\
	BFS3 (K = 2500, C = 15, depth = 50, Grid) & $\sim 0$ms & $\sim 2$s & $2.8 \pm 0.2$\\
	BFS3 (K = 5000, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 532$ms & $1.77 \pm 0.16$\\
	BFS3 (K = 5000, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 996$ms & $1.82 \pm 0.16$\\
	BFS3 (K = 5000, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 3$s & $1.96 \pm 0.18$\\
	BFS3 (K = 5000, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 500$ms & $2.98 \pm 0.2$\\
	BFS3 (K = 5000, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 1$s & $3.02 \pm 0.21$\\
	BFS3 (K = 5000, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 3$s & $3.18 \pm 0.22$\\
	BFS3 (K = 5000, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 738$ms & $2.46 \pm 0.2$\\
	BFS3 (K = 5000, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 1$s & $2.26 \pm 0.19$\\
	BFS3 (K = 5000, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 3$s & $2.45 \pm 0.19$\\
	BFS3 (K = 5000, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 876$ms & $2.49 \pm 0.18$\\
	BFS3 (K = 5000, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 2$s & $2.48 \pm 0.18$\\
	BFS3 (K = 5000, C = 15, depth = 50, Grid) & $\sim 0$ms & $\sim 5$s & $2.41 \pm 0.18$\\
	BFS3 (K = 10000, C = 2, depth = 15, Grid) & $\sim 0$ms & $\sim 1$s & $2.22 \pm 0.19$\\
	BFS3 (K = 10000, C = 2, depth = 25, Grid) & $\sim 0$ms & $\sim 2$s & $2.19 \pm 0.18$\\
	BFS3 (K = 10000, C = 2, depth = 50, Grid) & $\sim 0$ms & $\sim 5$s & $2.2 \pm 0.19$\\
	BFS3 (K = 10000, C = 5, depth = 15, Grid) & $\sim 0$ms & $\sim 829$ms & $3.18 \pm 0.23$\\
	BFS3 (K = 10000, C = 5, depth = 25, Grid) & $\sim 0$ms & $\sim 2$s & $3.18 \pm 0.22$\\
	BFS3 (K = 10000, C = 5, depth = 50, Grid) & $\sim 0$ms & $\sim 5$s & $3.22 \pm 0.23$\\
	BFS3 (K = 10000, C = 10, depth = 15, Grid) & $\sim 0$ms & $\sim 1$s & $2.42 \pm 0.19$\\
	BFS3 (K = 10000, C = 10, depth = 25, Grid) & $\sim 0$ms & $\sim 4$s & $2.48 \pm 0.19$\\
	BFS3 (K = 10000, C = 10, depth = 50, Grid) & $\sim 0$ms & $\sim 7$s & $2.37 \pm 0.2$\\
	BFS3 (K = 10000, C = 15, depth = 15, Grid) & $\sim 0$ms & $\sim 1$s & $2.29 \pm 0.18$\\
	BFS3 (K = 10000, C = 15, depth = 25, Grid) & $\sim 0$ms & $\sim 4$s & $2.3 \pm 0.19$\\
	SBOSS (epsilon = 1, delta = 9, Grid) & $\sim 0$ms & $\sim 0$ms & $4.2 \pm 0.31$\\
	SBOSS (epsilon = 1, delta = 7, Grid) & $\sim 0$ms & $\sim 0$ms & $4.12 \pm 0.3$\\
	SBOSS (epsilon = 1, delta = 5, Grid) & $\sim 0$ms & $\sim 0$ms & $4.18 \pm 0.31$\\
	SBOSS (epsilon = 1, delta = 3, Grid) & $\sim 0$ms & $\sim 0$ms & $3.96 \pm 0.32$\\
	SBOSS (epsilon = 1, delta = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.2 \pm 0.3$\\
	SBOSS (epsilon = 1, delta = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.26 \pm 0.31$\\
	SBOSS (epsilon = 1, delta = 0.01, Grid) & $\sim 0$ms & $\sim 0$ms & $4.2 \pm 0.32$\\
	SBOSS (epsilon = 1, delta = 0.001, Grid) & $\sim 0$ms & $\sim 0$ms & $4.17 \pm 0.32$\\
	SBOSS (epsilon = 0.1, delta = 9, Grid) & $\sim 0$ms & $\sim 0$ms & $4.17 \pm 0.32$\\
	\textbf{SBOSS (epsilon = 0.1, delta = 7, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{4.5 \pm 0.33}$\\
	SBOSS (epsilon = 0.1, delta = 5, Grid) & $\sim 0$ms & $\sim 0$ms & $4.33 \pm 0.32$\\
	SBOSS (epsilon = 0.1, delta = 3, Grid) & $\sim 0$ms & $\sim 0$ms & $4.1 \pm 0.32$\\
	SBOSS (epsilon = 0.1, delta = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.46 \pm 0.32$\\
	SBOSS (epsilon = 0.1, delta = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.27 \pm 0.32$\\
	SBOSS (epsilon = 0.1, delta = 0.01, Grid) & $\sim 0$ms & $\sim 0$ms & $4.43 \pm 0.31$\\
	SBOSS (epsilon = 0.1, delta = 0.001, Grid) & $\sim 0$ms & $\sim 0$ms & $4.25 \pm 0.3$\\
	SBOSS (epsilon = 0.01, delta = 9, Grid) & $\sim 0$ms & $\sim 0$ms & $4.26 \pm 0.3$\\
	SBOSS (epsilon = 0.01, delta = 7, Grid) & $\sim 0$ms & $\sim 0$ms & $4.16 \pm 0.31$\\
	SBOSS (epsilon = 0.01, delta = 5, Grid) & $\sim 0$ms & $\sim 0$ms & $4.2 \pm 0.32$\\
	SBOSS (epsilon = 0.01, delta = 3, Grid) & $\sim 0$ms & $\sim 0$ms & $4.25 \pm 0.31$\\
	SBOSS (epsilon = 0.01, delta = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.34 \pm 0.32$\\
	SBOSS (epsilon = 0.01, delta = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $3.98 \pm 0.31$\\
	SBOSS (epsilon = 0.01, delta = 0.01, Grid) & $\sim 0$ms & $\sim 0$ms & $4.18 \pm 0.33$\\
	SBOSS (epsilon = 0.01, delta = 0.001, Grid) & $\sim 0$ms & $\sim 0$ms & $4.26 \pm 0.32$\\
	SBOSS (epsilon = 0.001, delta = 9, Grid) & $\sim 0$ms & $\sim 0$ms & $4.19 \pm 0.32$\\
	SBOSS (epsilon = 0.001, delta = 7, Grid) & $\sim 0$ms & $\sim 0$ms & $4.36 \pm 0.32$\\
	SBOSS (epsilon = 0.001, delta = 5, Grid) & $\sim 0$ms & $\sim 0$ms & $4.27 \pm 0.32$\\
	SBOSS (epsilon = 0.001, delta = 3, Grid) & $\sim 0$ms & $\sim 0$ms & $4.26 \pm 0.33$\\
	SBOSS (epsilon = 0.001, delta = 1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.02 \pm 0.31$\\
	SBOSS (epsilon = 0.001, delta = 0.1, Grid) & $\sim 0$ms & $\sim 0$ms & $4.24 \pm 0.31$\\
	SBOSS (epsilon = 0.001, delta = 0.01, Grid) & $\sim 0$ms & $\sim 0$ms & $4.16 \pm 0.3$\\
	SBOSS (epsilon = 0.001, delta = 0.001, Grid) & $\sim 0$ms & $\sim 0$ms & $4.26 \pm 0.32$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, Grid) & $\sim 0$ms & $\sim 4$ms & $4.1 \pm 0.32$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, Grid) & $\sim 0$ms & $\sim 4$ms & $4.16 \pm 0.3$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, Grid) & $\sim 0$ms & $\sim 4$ms & $4.31 \pm 0.31$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, Grid) & $\sim 0$ms & $\sim 38$ms & $4.31 \pm 0.32$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, Grid) & $\sim 0$ms & $\sim 43$ms & $4.33 \pm 0.32$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, Grid) & $\sim 0$ms & $\sim 41$ms & $4.35 \pm 0.3$\\
	SBOSS (epsilon = 1e-06, delta = 0.0001, Grid) & $\sim 0$ms & $\sim 405$ms & $4.24 \pm 0.31$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, Grid) & $\sim 0$ms & $\sim 387$ms & $4.27 \pm 0.3$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, Grid) & $\sim 0$ms & $\sim 398$ms & $4.45 \pm 0.32$\\
	BEB (beta = 0.25, Grid) & $\sim 0$ms & $\sim 1$ms & $6.64 \pm 0.31$\\
	\textbf{BEB (beta = 0.5, Grid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{6.76 \pm 0.3}$\\
	BEB (beta = 1, Grid) & $\sim 0$ms & $\sim 1$ms & $6.24 \pm 0.28$\\
	BEB (beta = 1.5, Grid) & $\sim 0$ms & $\sim 1$ms & $6.48 \pm 0.31$\\
	BEB (beta = 2, Grid) & $\sim 0$ms & $\sim 1$ms & $5.71 \pm 0.29$\\
	BEB (beta = 2.5, Grid) & $\sim 0$ms & $\sim 1$ms & $5.71 \pm 0.29$\\
	BEB (beta = 3, Grid) & $\sim 0$ms & $\sim 1$ms & $4.07 \pm 0.23$\\
	BEB (beta = 4, Grid) & $\sim 0$ms & $\sim 1$ms & $3.01 \pm 0.2$\\
	BEB (beta = 8, Grid) & $\sim 0$ms & $\sim 1$ms & $1.63 \pm 0.14$\\
	BEB (beta = 16, Grid) & $\sim 0$ms & $\sim 1$ms & $0.99 \pm 0.11$\\
\end{longtable}


==> data/table-inaccurate-0.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{31.67 \pm 1.05}$\\
	\textbf{e-Greedy (e = 0, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.69 \pm 1.75}$\\
	e-Greedy (e = 0.1, UGC) & $\sim 0$ms & $\sim 0$ms & $37.2 \pm 1.51$\\
	e-Greedy (e = 0.2, UGC) & $\sim 0$ms & $\sim 0$ms & $35.72 \pm 1.4$\\
	e-Greedy (e = 0.3, UGC) & $\sim 0$ms & $\sim 0$ms & $34.74 \pm 1.28$\\
	e-Greedy (e = 0.4, UGC) & $\sim 0$ms & $\sim 0$ms & $34.58 \pm 1.33$\\
	e-Greedy (e = 0.5, UGC) & $\sim 0$ms & $\sim 0$ms & $34.91 \pm 1.31$\\
	e-Greedy (e = 0.6, UGC) & $\sim 0$ms & $\sim 0$ms & $32.75 \pm 1.08$\\
	e-Greedy (e = 0.7, UGC) & $\sim 0$ms & $\sim 0$ms & $32.21 \pm 1.02$\\
	e-Greedy (e = 0.8, UGC) & $\sim 0$ms & $\sim 0$ms & $31.96 \pm 1.02$\\
	e-Greedy (e = 0.9, UGC) & $\sim 0$ms & $\sim 0$ms & $32.05 \pm 1.03$\\
	e-Greedy (e = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $31.48 \pm 0.95$\\
	Soft-Max (tau = 0.05, UGC) & $\sim 0$ms & $\sim 0$ms & $34.14 \pm 1.75$\\
	Soft-Max (tau = 0.1, UGC) & $\sim 0$ms & $\sim 0$ms & $33.56 \pm 1.47$\\
	Soft-Max (tau = 0.2, UGC) & $\sim 0$ms & $\sim 0$ms & $33.61 \pm 1.52$\\
	\textbf{Soft-Max (tau = 0.33, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{34.75 \pm 1.64}$\\
	Soft-Max (tau = 0.5, UGC) & $\sim 0$ms & $\sim 0$ms & $34.75 \pm 1.64$\\
	Soft-Max (tau = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $33.81 \pm 1.6$\\
	Soft-Max (tau = 2, UGC) & $\sim 0$ms & $\sim 0$ms & $33.45 \pm 1.53$\\
	Soft-Max (tau = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $33.81 \pm 1.6$\\
	Soft-Max (tau = 5, UGC) & $\sim 0$ms & $\sim 0$ms & $34.02 \pm 1.5$\\
	Soft-Max (tau = 25, UGC) & $\sim 0$ms & $\sim 0$ms & $33.89 \pm 1.5$\\
	OPPS-DS (Formula (X0 ABS), UGC) & $\sim 838$ms & $\sim 0$ms & $38.42 \pm 1.71$\\
	OPPS-DS (Formula (X0 ABS), UGC) & $\sim 9$s & $\sim 0$ms & $37.23 \pm 1.59$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 21}$\textbf{s} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.74 \pm 1.76}$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 42}$\textbf{s} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.46 \pm 1.62}$\\
	OPPS-DS (Formula (X2 ABS), UGC) & $\sim 1$m & $\sim 0$ms & $37.56 \pm 1.6$\\
	OPPS-DS (Formula (X2), UGC) & $\sim 3$m & $\sim 0$ms & $37.46 \pm 1.62$\\
	OPPS-DS (Formula (X2 ABS), UGC) & $\sim 31$m & $\sim 0$ms & $36.93 \pm 1.6$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 5}$\textbf{h} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.68 \pm 1.55}$\\
	OPPS-DS (Formula (X2 X1 MUL2), UGC) & $\sim 1$s & $\sim 0$ms & $35.86 \pm 1.54$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 13}$\textbf{s} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.56 \pm 1.6}$\\
	OPPS-DS (Formula (X2 OPP INV), UGC) & $\sim 35$s & $\sim 0$ms & $38.39 \pm 1.68$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 1}$\textbf{m} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{39.29 \pm 1.71}$\\
	OPPS-DS (Formula (X1 X0 MIN2), UGC) & $\sim 2$m & $\sim 0$ms & $35.75 \pm 1.33$\\
	OPPS-DS (Formula (X0 OPP INV), UGC) & $\sim 5$m & $\sim 0$ms & $38.9 \pm 1.87$\\
	\textbf{OPPS-DS (Formula (X0), UGC)} & $\boldsymbol{\sim 47}$\textbf{m} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{37.32 \pm 1.6}$\\
	OPPS-DS (Formula (X2), UGC) & $\sim 8$h & $\sim 0$ms & $37.77 \pm 1.71$\\
	OPPS-DS (Formula (X2 X1 MAX2 INV), UGC) & $\sim 38$s & $\sim 0$ms & $30.42 \pm 0.94$\\
	OPPS-DS (Formula (X1 X0 MIN2), UGC) & $\sim 1$m & $\sim 0$ms & $36.83 \pm 1.77$\\
	OPPS-DS (Formula (X2 X0 INV SUB), UGC) & $\sim 3$m & $\sim 0$ms & $36.4 \pm 1.57$\\
	OPPS-DS (Formula (X2 OPP X0 MAX2), UGC) & $\sim 5$m & $\sim 0$ms & $39.12 \pm 1.82$\\
	OPPS-DS (Formula (X0 ABS LN ABS), UGC) & $\sim 50$m & $\sim 0$ms & $38.1 \pm 1.74$\\
	OPPS-DS (Formula (X2 X0 MIN2), UGC) & $\sim 8$h & $\sim 0$ms & $37.66 \pm 1.83$\\
	OPPS-DS (Formula (X2 X2 X0 MAX2 ADD2), UGC) & $\sim 42$s & $\sim 0$ms & $38.45 \pm 1.66$\\
	OPPS-DS (Formula (X2 INV X0 ABS ADD2), UGC) & $\sim 1$m & $\sim 0$ms & $38.45 \pm 1.66$\\
	OPPS-DS (Formula (X0 ABS SQRT X0 ADD2), UGC) & $\sim 3$m & $\sim 0$ms & $38.45 \pm 1.66$\\
	OPPS-DS (Formula (X2 X0 OPP MAX2), UGC) & $\sim 6$m & $\sim 0$ms & $38.58 \pm 1.84$\\
	OPPS-DS (Formula (X1 OPP X0 MAX2 ABS), UGC) & $\sim 56$m & $\sim 0$ms & $38.54 \pm 1.71$\\
	OPPS-DS (Formula (X2 X0 ABS OPP MAX2), UGC) & $\sim 9$h & $\sim 0$ms & $37.7 \pm 1.6$\\
	OPPS-DS (Formula (X2 X2 X1 MAX2 ADD2 ABS), UGC) & $\sim 5$m & $\sim 0$ms & $39.14 \pm 1.94$\\
	OPPS-DS (Formula (X2 X1 X0 ADD2 INV ADD2), UGC) & $\sim 6$m & $\sim 0$ms & $38.27 \pm 1.87$\\
	OPPS-DS (Formula (X1 ABS X2 SUB X0 ADD2), UGC) & $\sim 58$m & $\sim 0$ms & $34 \pm 1.3$\\
	OPPS-DS (Formula (X2 ABS LN X0 INV ADD2), UGC) & $\sim 9$h & $\sim 0$ms & $38.1 \pm 1.74$\\
	BAMCP (K = 1, depth = 15, UGC) & $\sim 0$ms & $\sim 0$ms & $31.77 \pm 1.02$\\
	BAMCP (K = 1, depth = 25, UGC) & $\sim 0$ms & $\sim 0$ms & $31.96 \pm 1.1$\\
	BAMCP (K = 1, depth = 50, UGC) & $\sim 0$ms & $\sim 0$ms & $31.64 \pm 0.97$\\
	BAMCP (K = 500, depth = 15, UGC) & $\sim 0$ms & $\sim 3$ms & $33.16 \pm 1.04$\\
	BAMCP (K = 500, depth = 25, UGC) & $\sim 0$ms & $\sim 3$ms & $32.24 \pm 1.04$\\
	BAMCP (K = 500, depth = 50, UGC) & $\sim 0$ms & $\sim 4$ms & $32.52 \pm 1.08$\\
	BAMCP (K = 1250, depth = 15, UGC) & $\sim 0$ms & $\sim 8$ms & $32.43 \pm 1.09$\\
	\textbf{BAMCP (K = 1250, depth = 25, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 8}$\textbf{ms} & $\boldsymbol{33.87 \pm 1.26}$\\
	BAMCP (K = 1250, depth = 50, UGC) & $\sim 0$ms & $\sim 10$ms & $32.83 \pm 1.09$\\
	BAMCP (K = 2500, depth = 15, UGC) & $\sim 0$ms & $\sim 15$ms & $32.57 \pm 1.11$\\
	BAMCP (K = 2500, depth = 25, UGC) & $\sim 0$ms & $\sim 16$ms & $32.24 \pm 1.09$\\
	BAMCP (K = 2500, depth = 50, UGC) & $\sim 0$ms & $\sim 22$ms & $32.15 \pm 1$\\
	BAMCP (K = 5000, depth = 15, UGC) & $\sim 0$ms & $\sim 30$ms & $33.17 \pm 1$\\
	BAMCP (K = 5000, depth = 25, UGC) & $\sim 0$ms & $\sim 46$ms & $33.23 \pm 1.12$\\
	BAMCP (K = 5000, depth = 50, UGC) & $\sim 0$ms & $\sim 42$ms & $33.86 \pm 1.23$\\
	BAMCP (K = 10000, depth = 15, UGC) & $\sim 0$ms & $\sim 60$ms & $33.48 \pm 1.2$\\
	BAMCP (K = 10000, depth = 25, UGC) & $\sim 0$ms & $\sim 106$ms & $33.28 \pm 1.14$\\
	BAMCP (K = 10000, depth = 50, UGC) & $\sim 0$ms & $\sim 85$ms & $32.89 \pm 1.08$\\
	BAMCP (K = 25000, depth = 15, UGC) & $\sim 0$ms & $\sim 156$ms & $33.19 \pm 1.25$\\
	BAMCP (K = 25000, depth = 25, UGC) & $\sim 0$ms & $\sim 293$ms & $32.55 \pm 1.11$\\
	BAMCP (K = 25000, depth = 50, UGC) & $\sim 0$ms & $\sim 214$ms & $31.98 \pm 0.98$\\
	BFS3 (K = 1, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 0$ms & $32.31 \pm 1.05$\\
	BFS3 (K = 1, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 0$ms & $33.31 \pm 1.21$\\
	BFS3 (K = 1, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 0$ms & $32.24 \pm 1.14$\\
	BFS3 (K = 1, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 1$ms & $33.03 \pm 1.3$\\
	BFS3 (K = 1, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 1$ms & $33.64 \pm 1.3$\\
	BFS3 (K = 1, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 2$ms & $34.19 \pm 1.38$\\
	BFS3 (K = 1, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 1$ms & $34.05 \pm 1.46$\\
	BFS3 (K = 1, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 2$ms & $34.77 \pm 1.51$\\
	BFS3 (K = 1, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 5$ms & $34.81 \pm 1.45$\\
	BFS3 (K = 1, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 2$ms & $35.45 \pm 1.41$\\
	BFS3 (K = 1, C = 15, depth = 25, UGC) & $\sim 0$ms & $\sim 4$ms & $35.26 \pm 1.61$\\
	BFS3 (K = 1, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 8$ms & $35.45 \pm 1.53$\\
	BFS3 (K = 500, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 24$ms & $32.91 \pm 1.25$\\
	BFS3 (K = 500, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 44$ms & $32.64 \pm 1.18$\\
	BFS3 (K = 500, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 118$ms & $33.21 \pm 1.16$\\
	BFS3 (K = 500, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 24$ms & $33.4 \pm 1.24$\\
	BFS3 (K = 500, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 48$ms & $33.85 \pm 1.21$\\
	BFS3 (K = 500, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 120$ms & $33.71 \pm 1.23$\\
	BFS3 (K = 500, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 39$ms & $36.17 \pm 1.56$\\
	BFS3 (K = 500, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 81$ms & $33.82 \pm 1.33$\\
	BFS3 (K = 500, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 173$ms & $34.47 \pm 1.27$\\
	BFS3 (K = 500, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 56$ms & $35.4 \pm 1.56$\\
	BFS3 (K = 500, C = 15, depth = 25, UGC) & $\sim 0$ms & $\sim 107$ms & $35.82 \pm 1.78$\\
	BFS3 (K = 500, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 221$ms & $35.57 \pm 1.59$\\
	BFS3 (K = 1250, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 59$ms & $33.81 \pm 1.28$\\
	BFS3 (K = 1250, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 112$ms & $32.68 \pm 1.12$\\
	BFS3 (K = 1250, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 285$ms & $32.78 \pm 1.27$\\
	BFS3 (K = 1250, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 38$ms & $33.63 \pm 1.29$\\
	BFS3 (K = 1250, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 78$ms & $33.47 \pm 1.22$\\
	BFS3 (K = 1250, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 213$ms & $33.25 \pm 1.12$\\
	BFS3 (K = 1250, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 63$ms & $33.92 \pm 1.36$\\
	BFS3 (K = 1250, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 138$ms & $35.37 \pm 1.41$\\
	BFS3 (K = 1250, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 352$ms & $35.09 \pm 1.4$\\
	BFS3 (K = 1250, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 102$ms & $36.86 \pm 1.67$\\
	\textbf{BFS3 (K = 1250, C = 15, depth = 25, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 196}$\textbf{ms} & $\boldsymbol{36.87 \pm 1.82}$\\
	BFS3 (K = 1250, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 472$ms & $35.74 \pm 1.64$\\
	BFS3 (K = 2500, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 126$ms & $32.18 \pm 1.11$\\
	BFS3 (K = 2500, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 400$ms & $32.56 \pm 1.04$\\
	BFS3 (K = 2500, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 542$ms & $32.26 \pm 1.13$\\
	BFS3 (K = 2500, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 53$ms & $32.66 \pm 1.09$\\
	BFS3 (K = 2500, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 185$ms & $33.29 \pm 1.26$\\
	BFS3 (K = 2500, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 318$ms & $33.77 \pm 1.28$\\
	BFS3 (K = 2500, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 133$ms & $35.48 \pm 1.47$\\
	BFS3 (K = 2500, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 188$ms & $35.86 \pm 1.64$\\
	BFS3 (K = 2500, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 980$ms & $34.55 \pm 1.43$\\
	BFS3 (K = 2500, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 186$ms & $35.3 \pm 1.47$\\
	BFS3 (K = 2500, C = 15, depth = 25, UGC) & $\sim 0$ms & $\sim 283$ms & $35.83 \pm 1.62$\\
	BFS3 (K = 2500, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 854$ms & $35.56 \pm 1.49$\\
	BFS3 (K = 5000, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 376$ms & $32.43 \pm 1.11$\\
	BFS3 (K = 5000, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 466$ms & $32.59 \pm 1.09$\\
	BFS3 (K = 5000, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 1$s & $32.17 \pm 1.04$\\
	BFS3 (K = 5000, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 89$ms & $33.4 \pm 1.18$\\
	BFS3 (K = 5000, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 168$ms & $34.27 \pm 1.38$\\
	BFS3 (K = 5000, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 464$ms & $32.7 \pm 1.04$\\
	BFS3 (K = 5000, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 122$ms & $34.83 \pm 1.59$\\
	BFS3 (K = 5000, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 418$ms & $34.71 \pm 1.45$\\
	BFS3 (K = 5000, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 861$ms & $34.82 \pm 1.44$\\
	BFS3 (K = 5000, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 172$ms & $35.83 \pm 1.54$\\
	BFS3 (K = 5000, C = 15, depth = 25, UGC) & $\sim 0$ms & $\sim 634$ms & $35.27 \pm 1.52$\\
	BFS3 (K = 5000, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 2$s & $35.9 \pm 1.7$\\
	BFS3 (K = 10000, C = 2, depth = 15, UGC) & $\sim 0$ms & $\sim 760$ms & $32.2 \pm 1.12$\\
	BFS3 (K = 10000, C = 2, depth = 25, UGC) & $\sim 0$ms & $\sim 897$ms & $32.47 \pm 1.04$\\
	BFS3 (K = 10000, C = 2, depth = 50, UGC) & $\sim 0$ms & $\sim 2$s & $32.26 \pm 1.04$\\
	BFS3 (K = 10000, C = 5, depth = 15, UGC) & $\sim 0$ms & $\sim 280$ms & $33.59 \pm 1.25$\\
	BFS3 (K = 10000, C = 5, depth = 25, UGC) & $\sim 0$ms & $\sim 503$ms & $33.2 \pm 1.17$\\
	BFS3 (K = 10000, C = 5, depth = 50, UGC) & $\sim 0$ms & $\sim 720$ms & $34.18 \pm 1.39$\\
	BFS3 (K = 10000, C = 10, depth = 15, UGC) & $\sim 0$ms & $\sim 213$ms & $34.49 \pm 1.55$\\
	BFS3 (K = 10000, C = 10, depth = 25, UGC) & $\sim 0$ms & $\sim 684$ms & $33.79 \pm 1.32$\\
	BFS3 (K = 10000, C = 10, depth = 50, UGC) & $\sim 0$ms & $\sim 1$s & $34.84 \pm 1.37$\\
	BFS3 (K = 10000, C = 15, depth = 15, UGC) & $\sim 0$ms & $\sim 266$ms & $36.72 \pm 1.81$\\
	BFS3 (K = 10000, C = 15, depth = 25, UGC) & $\sim 0$ms & $\sim 542$ms & $35.93 \pm 1.68$\\
	BFS3 (K = 10000, C = 15, depth = 50, UGC) & $\sim 0$ms & $\sim 2$s & $36.78 \pm 1.63$\\
	SBOSS (epsilon = 1, delta = 9, UGC) & $\sim 0$ms & $\sim 0$ms & $34.39 \pm 1.69$\\
	SBOSS (epsilon = 1, delta = 7, UGC) & $\sim 0$ms & $\sim 0$ms & $34.48 \pm 1.65$\\
	SBOSS (epsilon = 1, delta = 5, UGC) & $\sim 0$ms & $\sim 0$ms & $34.69 \pm 1.53$\\
	SBOSS (epsilon = 1, delta = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $34.8 \pm 1.56$\\
	SBOSS (epsilon = 1, delta = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $36.33 \pm 1.68$\\
	SBOSS (epsilon = 1, delta = 0.1, UGC) & $\sim 0$ms & $\sim 0$ms & $36.05 \pm 1.72$\\
	SBOSS (epsilon = 1, delta = 0.01, UGC) & $\sim 0$ms & $\sim 0$ms & $35.27 \pm 1.51$\\
	SBOSS (epsilon = 1, delta = 0.001, UGC) & $\sim 0$ms & $\sim 0$ms & $37.41 \pm 1.81$\\
	SBOSS (epsilon = 0.1, delta = 9, UGC) & $\sim 0$ms & $\sim 0$ms & $34 \pm 1.66$\\
	SBOSS (epsilon = 0.1, delta = 7, UGC) & $\sim 0$ms & $\sim 0$ms & $32.51 \pm 1.44$\\
	SBOSS (epsilon = 0.1, delta = 5, UGC) & $\sim 0$ms & $\sim 0$ms & $34.13 \pm 1.5$\\
	SBOSS (epsilon = 0.1, delta = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $34.98 \pm 1.61$\\
	SBOSS (epsilon = 0.1, delta = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $37.26 \pm 1.81$\\
	SBOSS (epsilon = 0.1, delta = 0.1, UGC) & $\sim 0$ms & $\sim 0$ms & $36.3 \pm 1.77$\\
	SBOSS (epsilon = 0.1, delta = 0.01, UGC) & $\sim 0$ms & $\sim 0$ms & $35.21 \pm 1.52$\\
	SBOSS (epsilon = 0.1, delta = 0.001, UGC) & $\sim 0$ms & $\sim 0$ms & $35.21 \pm 1.52$\\
	SBOSS (epsilon = 0.01, delta = 9, UGC) & $\sim 0$ms & $\sim 0$ms & $34.84 \pm 1.51$\\
	SBOSS (epsilon = 0.01, delta = 7, UGC) & $\sim 0$ms & $\sim 0$ms & $34.39 \pm 1.55$\\
	SBOSS (epsilon = 0.01, delta = 5, UGC) & $\sim 0$ms & $\sim 0$ms & $35.17 \pm 1.46$\\
	SBOSS (epsilon = 0.01, delta = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $35.3 \pm 1.57$\\
	SBOSS (epsilon = 0.01, delta = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $35.63 \pm 1.49$\\
	SBOSS (epsilon = 0.01, delta = 0.1, UGC) & $\sim 0$ms & $\sim 0$ms & $37.11 \pm 1.73$\\
	SBOSS (epsilon = 0.01, delta = 0.01, UGC) & $\sim 0$ms & $\sim 0$ms & $35.78 \pm 1.61$\\
	SBOSS (epsilon = 0.01, delta = 0.001, UGC) & $\sim 0$ms & $\sim 0$ms & $35.94 \pm 1.67$\\
	SBOSS (epsilon = 0.001, delta = 9, UGC) & $\sim 0$ms & $\sim 0$ms & $33.89 \pm 1.64$\\
	SBOSS (epsilon = 0.001, delta = 7, UGC) & $\sim 0$ms & $\sim 0$ms & $33 \pm 1.5$\\
	SBOSS (epsilon = 0.001, delta = 5, UGC) & $\sim 0$ms & $\sim 0$ms & $35.1 \pm 1.64$\\
	SBOSS (epsilon = 0.001, delta = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $37.44 \pm 1.9$\\
	SBOSS (epsilon = 0.001, delta = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $36.7 \pm 1.72$\\
	SBOSS (epsilon = 0.001, delta = 0.1, UGC) & $\sim 0$ms & $\sim 1$ms & $35.88 \pm 1.58$\\
	SBOSS (epsilon = 0.001, delta = 0.01, UGC) & $\sim 0$ms & $\sim 1$ms & $37.56 \pm 1.77$\\
	SBOSS (epsilon = 0.001, delta = 0.001, UGC) & $\sim 0$ms & $\sim 1$ms & $38.49 \pm 2.04$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, UGC) & $\sim 0$ms & $\sim 9$ms & $38.58 \pm 1.96$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, UGC) & $\sim 0$ms & $\sim 9$ms & $37.32 \pm 1.79$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, UGC) & $\sim 0$ms & $\sim 9$ms & $37.14 \pm 1.76$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, UGC) & $\sim 0$ms & $\sim 94$ms & $36.43 \pm 1.68$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, UGC) & $\sim 0$ms & $\sim 192$ms & $38.02 \pm 1.71$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, UGC) & $\sim 0$ms & $\sim 107$ms & $36.29 \pm 1.64$\\
	\textbf{SBOSS (epsilon = 1e-06, delta = 0.0001, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{s} & $\boldsymbol{38.77 \pm 1.89}$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, UGC) & $\sim 0$ms & $\sim 1$s & $36.84 \pm 1.78$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, UGC) & $\sim 0$ms & $\sim 1$s & $37.13 \pm 1.75$\\
	BEB (beta = 0.25, UGC) & $\sim 0$ms & $\sim 0$ms & $37.54 \pm 1.63$\\
	BEB (beta = 0.5, UGC) & $\sim 0$ms & $\sim 0$ms & $37.23 \pm 1.6$\\
	BEB (beta = 1, UGC) & $\sim 0$ms & $\sim 0$ms & $37.63 \pm 1.75$\\
	BEB (beta = 1.5, UGC) & $\sim 0$ms & $\sim 0$ms & $37.8 \pm 1.52$\\
	BEB (beta = 2, UGC) & $\sim 0$ms & $\sim 0$ms & $37.53 \pm 1.66$\\
	BEB (beta = 2.5, UGC) & $\sim 0$ms & $\sim 0$ms & $36.23 \pm 1.47$\\
	BEB (beta = 3, UGC) & $\sim 0$ms & $\sim 0$ms & $36.68 \pm 1.58$\\
	BEB (beta = 4, UGC) & $\sim 0$ms & $\sim 0$ms & $37.35 \pm 1.52$\\
	BEB (beta = 8, UGC) & $\sim 0$ms & $\sim 0$ms & $38.19 \pm 1.73$\\
	\textbf{BEB (beta = 16, UGC)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{38.34 \pm 1.62}$\\
\end{longtable}


==> data/table-inaccurate-1.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.76 \pm 0.08}$\\
	e-Greedy (e = 0, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.85 \pm 0.07$\\
	e-Greedy (e = 0.1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.87 \pm 0.08$\\
	e-Greedy (e = 0.2, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.83 \pm 0.07$\\
	\textbf{e-Greedy (e = 0.3, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.88 \pm 0.07}$\\
	e-Greedy (e = 0.4, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.83 \pm 0.07$\\
	e-Greedy (e = 0.5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.85 \pm 0.08$\\
	e-Greedy (e = 0.6, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.07$\\
	e-Greedy (e = 0.7, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.08$\\
	e-Greedy (e = 0.8, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	e-Greedy (e = 0.9, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.08$\\
	e-Greedy (e = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	\textbf{Soft-Max (tau = 0.05, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.76 \pm 0.1}$\\
	Soft-Max (tau = 0.1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.1$\\
	Soft-Max (tau = 0.2, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.1$\\
	Soft-Max (tau = 0.33, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.1$\\
	Soft-Max (tau = 0.5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.73 \pm 0.1$\\
	Soft-Max (tau = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	Soft-Max (tau = 2, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.1$\\
	Soft-Max (tau = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.1$\\
	Soft-Max (tau = 5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.7 \pm 0.1$\\
	Soft-Max (tau = 25, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.74 \pm 0.1$\\
	OPPS-DS (Formula (X2), UGDL) & $\sim 519$ms & $\sim 0$ms & $2.84 \pm 0.08$\\
	OPPS-DS (Formula (X1 ABS), UGDL) & $\sim 5$s & $\sim 0$ms & $2.9 \pm 0.08$\\
	OPPS-DS (Formula (X1 ABS), UGDL) & $\sim 12$s & $\sim 0$ms & $2.86 \pm 0.08$\\
	OPPS-DS (Formula (X2 ABS), UGDL) & $\sim 24$s & $\sim 0$ms & $2.9 \pm 0.07$\\
	OPPS-DS (Formula (X2 ABS), UGDL) & $\sim 47$s & $\sim 0$ms & $2.85 \pm 0.07$\\
	OPPS-DS (Formula (X2 ABS), UGDL) & $\sim 2$m & $\sim 0$ms & $2.83 \pm 0.07$\\
	OPPS-DS (Formula (X2 ABS), UGDL) & $\sim 16$m & $\sim 0$ms & $2.86 \pm 0.07$\\
	OPPS-DS (Formula (X0), UGDL) & $\sim 2$h & $\sim 0$ms & $2.83 \pm 0.07$\\
	OPPS-DS (Formula (X2 ABS), UGDL) & $\sim 741$ms & $\sim 0$ms & $2.82 \pm 0.07$\\
	OPPS-DS (Formula (X1 X0 SUB), UGDL) & $\sim 7$s & $\sim 0$ms & $2.66 \pm 0.1$\\
	\textbf{OPPS-DS (Formula (X1 X0 MAX2), UGDL)} & $\boldsymbol{\sim 19}$\textbf{s} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.99 \pm 0.08}$\\
	OPPS-DS (Formula (X2 X0 ADD2), UGDL) & $\sim 37$s & $\sim 0$ms & $2.82 \pm 0.07$\\
	OPPS-DS (Formula (X1 ABS), UGDL) & $\sim 1$m & $\sim 0$ms & $2.88 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 MUL2), UGDL) & $\sim 2$m & $\sim 0$ms & $2.88 \pm 0.08$\\
	OPPS-DS (Formula (X0 ABS), UGDL) & $\sim 23$m & $\sim 0$ms & $2.82 \pm 0.07$\\
	OPPS-DS (Formula (X2 OPP INV), UGDL) & $\sim 4$h & $\sim 0$ms & $2.9 \pm 0.07$\\
	OPPS-DS (Formula (X2 INV ABS), UGDL) & $\sim 20$s & $\sim 0$ms & $2.66 \pm 0.1$\\
	OPPS-DS (Formula (X1 X0 MUL2), UGDL) & $\sim 39$s & $\sim 0$ms & $2.85 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 SUB), UGDL) & $\sim 1$m & $\sim 0$ms & $2.69 \pm 0.09$\\
	OPPS-DS (Formula (X2 X1 ABS ADD2), UGDL) & $\sim 3$m & $\sim 0$ms & $2.95 \pm 0.08$\\
	OPPS-DS (Formula (X1 ABS X0 ADD2), UGDL) & $\sim 25$m & $\sim 0$ms & $2.92 \pm 0.08$\\
	OPPS-DS (Formula (X2 ABS X0 ADD2), UGDL) & $\sim 4$h & $\sim 0$ms & $2.86 \pm 0.07$\\
	OPPS-DS (Formula (X1 X1 X0 MIN2 SUB), UGDL) & $\sim 22$s & $\sim 0$ms & $2.89 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 ABS DIV), UGDL) & $\sim 45$s & $\sim 0$ms & $2.9 \pm 0.08$\\
	OPPS-DS (Formula (X2 X1 SUB X1 MAX2), UGDL) & $\sim 1$m & $\sim 0$ms & $2.95 \pm 0.08$\\
	OPPS-DS (Formula (X0 ABS X0 SUB), UGDL) & $\sim 3$m & $\sim 0$ms & $2.78 \pm 0.07$\\
	OPPS-DS (Formula (X1 X0 X0 MUL2 MIN2), UGDL) & $\sim 32$m & $\sim 0$ms & $2.79 \pm 0.07$\\
	OPPS-DS (Formula (X0 X2 DIV X0 MUL2), UGDL) & $\sim 5$h & $\sim 0$ms & $2.82 \pm 0.07$\\
	OPPS-DS (Formula (X1 X0 SUB X0 MUL2 ABS), UGDL) & $\sim 2$m & $\sim 0$ms & $2.96 \pm 0.07$\\
	OPPS-DS (Formula (X0 INV ABS X2 ABS SUB), UGDL) & $\sim 3$m & $\sim 0$ms & $2.59 \pm 0.09$\\
	OPPS-DS (Formula (X1 ABS X1 X2 DIV SUB), UGDL) & $\sim 31$m & $\sim 0$ms & $2.83 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 ABS X0 ADD2 MIN2), UGDL) & $\sim 5$h & $\sim 0$ms & $2.86 \pm 0.07$\\
	BAMCP (K = 1, depth = 15, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.69 \pm 0.08$\\
	BAMCP (K = 1, depth = 25, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.77 \pm 0.08$\\
	BAMCP (K = 1, depth = 50, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.73 \pm 0.08$\\
	BAMCP (K = 500, depth = 15, UGDL) & $\sim 0$ms & $\sim 5$ms & $2.78 \pm 0.08$\\
	BAMCP (K = 500, depth = 25, UGDL) & $\sim 0$ms & $\sim 5$ms & $2.75 \pm 0.07$\\
	BAMCP (K = 500, depth = 50, UGDL) & $\sim 0$ms & $\sim 6$ms & $2.78 \pm 0.07$\\
	BAMCP (K = 1250, depth = 15, UGDL) & $\sim 0$ms & $\sim 12$ms & $2.76 \pm 0.08$\\
	BAMCP (K = 1250, depth = 25, UGDL) & $\sim 0$ms & $\sim 13$ms & $2.79 \pm 0.07$\\
	BAMCP (K = 1250, depth = 50, UGDL) & $\sim 0$ms & $\sim 16$ms & $2.79 \pm 0.08$\\
	BAMCP (K = 2500, depth = 15, UGDL) & $\sim 0$ms & $\sim 26$ms & $2.78 \pm 0.07$\\
	BAMCP (K = 2500, depth = 25, UGDL) & $\sim 0$ms & $\sim 28$ms & $2.79 \pm 0.08$\\
	BAMCP (K = 2500, depth = 50, UGDL) & $\sim 0$ms & $\sim 31$ms & $2.8 \pm 0.08$\\
	BAMCP (K = 5000, depth = 15, UGDL) & $\sim 0$ms & $\sim 50$ms & $2.81 \pm 0.07$\\
	BAMCP (K = 5000, depth = 25, UGDL) & $\sim 0$ms & $\sim 54$ms & $2.83 \pm 0.07$\\
	BAMCP (K = 5000, depth = 50, UGDL) & $\sim 0$ms & $\sim 96$ms & $2.8 \pm 0.08$\\
	BAMCP (K = 10000, depth = 15, UGDL) & $\sim 0$ms & $\sim 100$ms & $2.82 \pm 0.07$\\
	BAMCP (K = 10000, depth = 25, UGDL) & $\sim 0$ms & $\sim 115$ms & $2.79 \pm 0.07$\\
	\textbf{BAMCP (K = 10000, depth = 50, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 207}$\textbf{ms} & $\boldsymbol{2.85 \pm 0.07}$\\
	BAMCP (K = 25000, depth = 15, UGDL) & $\sim 0$ms & $\sim 426$ms & $2.85 \pm 0.07$\\
	BAMCP (K = 25000, depth = 25, UGDL) & $\sim 0$ms & $\sim 278$ms & $2.8 \pm 0.07$\\
	BAMCP (K = 25000, depth = 50, UGDL) & $\sim 0$ms & $\sim 322$ms & $2.84 \pm 0.07$\\
	BFS3 (K = 1, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.08$\\
	BFS3 (K = 1, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 1, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.73 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.08$\\
	BFS3 (K = 1, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.77 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 1, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 3$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 1, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 2$ms & $2.77 \pm 0.07$\\
	BFS3 (K = 1, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 3$ms & $2.8 \pm 0.07$\\
	BFS3 (K = 1, C = 15, depth = 50, UGDL) & $\sim 0$ms & $\sim 5$ms & $2.81 \pm 0.07$\\
	BFS3 (K = 500, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 15$ms & $2.76 \pm 0.07$\\
	BFS3 (K = 500, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 26$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 500, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 60$ms & $2.77 \pm 0.08$\\
	BFS3 (K = 500, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 13$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 500, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 29$ms & $2.79 \pm 0.08$\\
	BFS3 (K = 500, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 82$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 500, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 24$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 500, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 51$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 500, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 125$ms & $2.81 \pm 0.07$\\
	BFS3 (K = 500, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 33$ms & $2.8 \pm 0.08$\\
	BFS3 (K = 500, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 72$ms & $2.76 \pm 0.07$\\
	BFS3 (K = 500, C = 15, depth = 50, UGDL) & $\sim 0$ms & $\sim 164$ms & $2.82 \pm 0.07$\\
	BFS3 (K = 1250, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 34$ms & $2.83 \pm 0.07$\\
	BFS3 (K = 1250, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 62$ms & $2.81 \pm 0.07$\\
	BFS3 (K = 1250, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 142$ms & $2.77 \pm 0.08$\\
	BFS3 (K = 1250, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 20$ms & $2.8 \pm 0.07$\\
	BFS3 (K = 1250, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 44$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 1250, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 133$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 1250, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 32$ms & $2.85 \pm 0.07$\\
	BFS3 (K = 1250, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 74$ms & $2.79 \pm 0.08$\\
	BFS3 (K = 1250, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 224$ms & $2.84 \pm 0.07$\\
	BFS3 (K = 1250, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 43$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 1250, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 107$ms & $2.77 \pm 0.07$\\
	\textbf{BFS3 (K = 1250, C = 15, depth = 50, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 329}$\textbf{ms} & $\boldsymbol{2.85 \pm 0.07}$\\
	BFS3 (K = 2500, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 111$ms & $2.85 \pm 0.07$\\
	BFS3 (K = 2500, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 131$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 2500, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 292$ms & $2.77 \pm 0.08$\\
	BFS3 (K = 2500, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 32$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 2500, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 89$ms & $2.8 \pm 0.08$\\
	BFS3 (K = 2500, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 219$ms & $2.8 \pm 0.08$\\
	BFS3 (K = 2500, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 70$ms & $2.79 \pm 0.08$\\
	BFS3 (K = 2500, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 145$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 2500, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 484$ms & $2.74 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 58$ms & $2.84 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 132$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 50, UGDL) & $\sim 0$ms & $\sim 438$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 5000, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 128$ms & $2.73 \pm 0.08$\\
	BFS3 (K = 5000, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 248$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 5000, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 604$ms & $2.72 \pm 0.07$\\
	BFS3 (K = 5000, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 89$ms & $2.72 \pm 0.08$\\
	BFS3 (K = 5000, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 99$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 5000, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 243$ms & $2.77 \pm 0.07$\\
	BFS3 (K = 5000, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 71$ms & $2.82 \pm 0.07$\\
	BFS3 (K = 5000, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 135$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 5000, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 555$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 5000, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 88$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 5000, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 284$ms & $2.81 \pm 0.08$\\
	BFS3 (K = 5000, C = 15, depth = 50, UGDL) & $\sim 0$ms & $\sim 547$ms & $2.8 \pm 0.07$\\
	BFS3 (K = 10000, C = 2, depth = 15, UGDL) & $\sim 0$ms & $\sim 321$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 10000, C = 2, depth = 25, UGDL) & $\sim 0$ms & $\sim 498$ms & $2.75 \pm 0.07$\\
	BFS3 (K = 10000, C = 2, depth = 50, UGDL) & $\sim 0$ms & $\sim 1$s & $2.74 \pm 0.07$\\
	BFS3 (K = 10000, C = 5, depth = 15, UGDL) & $\sim 0$ms & $\sim 99$ms & $2.81 \pm 0.08$\\
	BFS3 (K = 10000, C = 5, depth = 25, UGDL) & $\sim 0$ms & $\sim 178$ms & $2.73 \pm 0.07$\\
	BFS3 (K = 10000, C = 5, depth = 50, UGDL) & $\sim 0$ms & $\sim 409$ms & $2.78 \pm 0.07$\\
	BFS3 (K = 10000, C = 10, depth = 15, UGDL) & $\sim 0$ms & $\sim 122$ms & $2.83 \pm 0.07$\\
	BFS3 (K = 10000, C = 10, depth = 25, UGDL) & $\sim 0$ms & $\sim 211$ms & $2.8 \pm 0.07$\\
	BFS3 (K = 10000, C = 10, depth = 50, UGDL) & $\sim 0$ms & $\sim 564$ms & $2.78 \pm 0.08$\\
	BFS3 (K = 10000, C = 15, depth = 15, UGDL) & $\sim 0$ms & $\sim 147$ms & $2.79 \pm 0.07$\\
	BFS3 (K = 10000, C = 15, depth = 25, UGDL) & $\sim 0$ms & $\sim 276$ms & $2.82 \pm 0.07$\\
	BFS3 (K = 10000, C = 15, depth = 50, UGDL) & $\sim 0$ms & $\sim 754$ms & $2.78 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 9, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.74 \pm 0.09$\\
	SBOSS (epsilon = 1, delta = 7, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.08$\\
	SBOSS (epsilon = 1, delta = 5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.08$\\
	SBOSS (epsilon = 1, delta = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 0.1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.77 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 0.01, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 0.001, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	SBOSS (epsilon = 0.1, delta = 9, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.08$\\
	SBOSS (epsilon = 0.1, delta = 7, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.08$\\
	SBOSS (epsilon = 0.1, delta = 5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.08$\\
	SBOSS (epsilon = 0.1, delta = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.07$\\
	SBOSS (epsilon = 0.1, delta = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.83 \pm 0.07$\\
	SBOSS (epsilon = 0.1, delta = 0.1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.76 \pm 0.08$\\
	SBOSS (epsilon = 0.1, delta = 0.01, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.07$\\
	\textbf{SBOSS (epsilon = 0.1, delta = 0.001, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.86 \pm 0.07}$\\
	SBOSS (epsilon = 0.01, delta = 9, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.71 \pm 0.09$\\
	SBOSS (epsilon = 0.01, delta = 7, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.74 \pm 0.09$\\
	SBOSS (epsilon = 0.01, delta = 5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.08$\\
	SBOSS (epsilon = 0.01, delta = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.08$\\
	SBOSS (epsilon = 0.01, delta = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.08$\\
	SBOSS (epsilon = 0.01, delta = 0.1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.08$\\
	SBOSS (epsilon = 0.01, delta = 0.01, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.08$\\
	SBOSS (epsilon = 0.01, delta = 0.001, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.8 \pm 0.07$\\
	SBOSS (epsilon = 0.001, delta = 9, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.73 \pm 0.09$\\
	SBOSS (epsilon = 0.001, delta = 7, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.75 \pm 0.08$\\
	SBOSS (epsilon = 0.001, delta = 5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.72 \pm 0.08$\\
	SBOSS (epsilon = 0.001, delta = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.81 \pm 0.08$\\
	SBOSS (epsilon = 0.001, delta = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.78 \pm 0.07$\\
	SBOSS (epsilon = 0.001, delta = 0.1, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.81 \pm 0.07$\\
	SBOSS (epsilon = 0.001, delta = 0.01, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.82 \pm 0.08$\\
	SBOSS (epsilon = 0.001, delta = 0.001, UGDL) & $\sim 0$ms & $\sim 1$ms & $2.81 \pm 0.07$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, UGDL) & $\sim 0$ms & $\sim 7$ms & $2.8 \pm 0.07$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, UGDL) & $\sim 0$ms & $\sim 7$ms & $2.83 \pm 0.07$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, UGDL) & $\sim 0$ms & $\sim 7$ms & $2.82 \pm 0.07$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, UGDL) & $\sim 0$ms & $\sim 68$ms & $2.85 \pm 0.08$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, UGDL) & $\sim 0$ms & $\sim 78$ms & $2.82 \pm 0.07$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, UGDL) & $\sim 0$ms & $\sim 78$ms & $2.81 \pm 0.08$\\
	SBOSS (epsilon = 1e-06, delta = 0.0001, UGDL) & $\sim 0$ms & $\sim 1$s & $2.83 \pm 0.07$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, UGDL) & $\sim 0$ms & $\sim 929$ms & $2.76 \pm 0.07$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, UGDL) & $\sim 0$ms & $\sim 1$s & $2.81 \pm 0.07$\\
	BEB (beta = 0.25, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.86 \pm 0.07$\\
	BEB (beta = 0.5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.87 \pm 0.07$\\
	BEB (beta = 1, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.85 \pm 0.07$\\
	BEB (beta = 1.5, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.84 \pm 0.07$\\
	BEB (beta = 2, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.86 \pm 0.07$\\
	\textbf{BEB (beta = 2.5, UGDL)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{2.88 \pm 0.07}$\\
	BEB (beta = 3, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.86 \pm 0.08$\\
	BEB (beta = 4, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.79 \pm 0.08$\\
	BEB (beta = 8, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.82 \pm 0.07$\\
	BEB (beta = 16, UGDL) & $\sim 0$ms & $\sim 0$ms & $2.83 \pm 0.07$\\
\end{longtable}


==> data/table-inaccurate-2.tex <==
\begin{longtable}{l|l|l|l}
	Agent & Offline time & Mean online time (per decision) & Score\\
	\hline
	\textbf{Random} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{0.23 \pm 0.06}$\\
	e-Greedy (e = 0, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.56 \pm 0.09$\\
	e-Greedy (e = 0.1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.58 \pm 0.09$\\
	\textbf{e-Greedy (e = 0.2, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{0.63 \pm 0.09}$\\
	e-Greedy (e = 0.3, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.43 \pm 0.07$\\
	e-Greedy (e = 0.4, UGrid) & $\sim 1$ms & $\sim 1$ms & $0.56 \pm 0.09$\\
	e-Greedy (e = 0.5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.43 \pm 0.08$\\
	e-Greedy (e = 0.6, UGrid) & $\sim 1$ms & $\sim 1$ms & $0.45 \pm 0.08$\\
	e-Greedy (e = 0.7, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.37 \pm 0.07$\\
	e-Greedy (e = 0.8, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.35 \pm 0.07$\\
	e-Greedy (e = 0.9, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.25 \pm 0.06$\\
	e-Greedy (e = 1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.21 \pm 0.05$\\
	\textbf{Soft-Max (tau = 0.05, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{0 \pm 0}$\\
	Soft-Max (tau = 0.1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.2, UGrid) & $\sim 1$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.33, UGrid) & $\sim 1$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 0.5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 2, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 3, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	Soft-Max (tau = 25, UGrid) & $\sim 0$ms & $\sim 1$ms & $0 \pm 0$\\
	OPPS-DS (Formula (X2), UGrid) & $\sim 6$s & $\sim 1$ms & $0.64 \pm 0.1$\\
	OPPS-DS (Formula (X0), UGrid) & $\sim 57$s & $\sim 1$ms & $0.6 \pm 0.09$\\
	OPPS-DS (Formula (X2 ABS), UGrid) & $\sim 3$m & $\sim 1$ms & $0.6 \pm 0.09$\\
	OPPS-DS (Formula (X2 ABS), UGrid) & $\sim 5$m & $\sim 1$ms & $0.65 \pm 0.1$\\
	OPPS-DS (Formula (X2), UGrid) & $\sim 10$m & $\sim 1$ms & $0.56 \pm 0.09$\\
	OPPS-DS (Formula (X0), UGrid) & $\sim 20$m & $\sim 1$ms & $0.65 \pm 0.09$\\
	OPPS-DS (Formula (X0 ABS), UGrid) & $\sim 3$h & $\sim 1$ms & $0.61 \pm 0.1$\\
	OPPS-DS (Formula (X0 ABS), UGrid) & $\sim 1$d & $\sim 1$ms & $0.68 \pm 0.1$\\
	OPPS-DS (Formula (X1), UGrid) & $\sim 9$s & $\sim 0$ms & $0.35 \pm 0.09$\\
	\textbf{OPPS-DS (Formula (X2 X1 ADD2), UGrid)} & $\boldsymbol{\sim 2}$\textbf{m} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{1.09 \pm 0.17}$\\
	OPPS-DS (Formula (X2 OPP INV), UGrid) & $\sim 4$m & $\sim 1$ms & $0.6 \pm 0.09$\\
	OPPS-DS (Formula (X2 X1 MUL2), UGrid) & $\sim 8$m & $\sim 1$ms & $0.43 \pm 0.11$\\
	OPPS-DS (Formula (X2 X1 SUB), UGrid) & $\sim 15$m & $\sim 1$ms & $0.53 \pm 0.08$\\
	OPPS-DS (Formula (X2 OPP INV), UGrid) & $\sim 32$m & $\sim 1$ms & $0.54 \pm 0.08$\\
	OPPS-DS (Formula (X2), UGrid) & $\sim 5$h & $\sim 1$ms & $0.57 \pm 0.08$\\
	OPPS-DS (Formula (X1 X0 MAX2), UGrid) & $\sim 2$d & $\sim 1$ms & $0.96 \pm 0.16$\\
	OPPS-DS (Formula (X1 X0 OPP MAX2), UGrid) & $\sim 4$m & $\sim 1$ms & $0.33 \pm 0.09$\\
	OPPS-DS (Formula (X1 OPP X0 DIV), UGrid) & $\sim 8$m & $\sim 1$ms & $0.2 \pm 0.05$\\
	OPPS-DS (Formula (X2 X0 ABS MIN2), UGrid) & $\sim 17$m & $\sim 2$ms & $0.58 \pm 0.08$\\
	OPPS-DS (Formula (X0 INV X0 MIN2), UGrid) & $\sim 33$m & $\sim 1$ms & $0.53 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 OPP MAX2), UGrid) & $\sim 6$h & $\sim 2$ms & $0.56 \pm 0.08$\\
	OPPS-DS (Formula (X2 ABS), UGrid) & $\sim 2$d & $\sim 1$ms & $0.56 \pm 0.08$\\
	OPPS-DS (Formula (X2 X1 X2 DIV MAX2), UGrid) & $\sim 5$m & $\sim 1$ms & $0.6 \pm 0.09$\\
	OPPS-DS (Formula (X2 X2 X1 SUB MAX2), UGrid) & $\sim 10$m & $\sim 1$ms & $0.61 \pm 0.09$\\
	OPPS-DS (Formula (X2 ABS X2 ADD2), UGrid) & $\sim 20$m & $\sim 1$ms & $0.59 \pm 0.09$\\
	OPPS-DS (Formula (X0 OPP INV X0 SUB), UGrid) & $\sim 39$m & $\sim 1$ms & $0.55 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 MAX2 X0 MUL2), UGrid) & $\sim 6$h & $\sim 2$ms & $0.56 \pm 0.09$\\
	OPPS-DS (Formula (X1 X1 ADD2 X0 ADD2), UGrid) & $\sim 3$d & $\sim 1$ms & $0.83 \pm 0.14$\\
	OPPS-DS (Formula (X1 X0 X0 MUL2 SUB INV), UGrid) & $\sim 31$m & $\sim 1$ms & $0.55 \pm 0.08$\\
	OPPS-DS (Formula (X2 X0 ADD2 X0 ABS MUL2), UGrid) & $\sim 39$m & $\sim 2$ms & $0.62 \pm 0.09$\\
	OPPS-DS (Formula (X2 X2 MUL2 X1 ADD2), UGrid) & $\sim 7$h & $\sim 1$ms & $1.03 \pm 0.15$\\
	OPPS-DS (Formula (X2 X1 MAX2 X0 ADD2), UGrid) & $\sim 3$d & $\sim 2$ms & $1.03 \pm 0.15$\\
	BAMCP (K = 1, depth = 15, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.23 \pm 0.05$\\
	BAMCP (K = 1, depth = 25, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.21 \pm 0.05$\\
	BAMCP (K = 1, depth = 50, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.18 \pm 0.04$\\
	BAMCP (K = 500, depth = 15, UGrid) & $\sim 0$ms & $\sim 64$ms & $0.43 \pm 0.07$\\
	BAMCP (K = 500, depth = 25, UGrid) & $\sim 0$ms & $\sim 64$ms & $0.39 \pm 0.07$\\
	BAMCP (K = 500, depth = 50, UGrid) & $\sim 0$ms & $\sim 66$ms & $0.48 \pm 0.08$\\
	BAMCP (K = 1250, depth = 15, UGrid) & $\sim 0$ms & $\sim 159$ms & $0.42 \pm 0.08$\\
	BAMCP (K = 1250, depth = 25, UGrid) & $\sim 0$ms & $\sim 160$ms & $0.49 \pm 0.08$\\
	BAMCP (K = 1250, depth = 50, UGrid) & $\sim 0$ms & $\sim 165$ms & $0.43 \pm 0.08$\\
	BAMCP (K = 2500, depth = 15, UGrid) & $\sim 0$ms & $\sim 331$ms & $0.5 \pm 0.09$\\
	BAMCP (K = 2500, depth = 25, UGrid) & $\sim 0$ms & $\sim 332$ms & $0.46 \pm 0.08$\\
	BAMCP (K = 2500, depth = 50, UGrid) & $\sim 0$ms & $\sim 363$ms & $0.46 \pm 0.08$\\
	BAMCP (K = 5000, depth = 15, UGrid) & $\sim 0$ms & $\sim 647$ms & $0.46 \pm 0.09$\\
	BAMCP (K = 5000, depth = 25, UGrid) & $\sim 0$ms & $\sim 669$ms & $0.5 \pm 0.09$\\
	BAMCP (K = 5000, depth = 50, UGrid) & $\sim 0$ms & $\sim 669$ms & $0.46 \pm 0.08$\\
	BAMCP (K = 10000, depth = 15, UGrid) & $\sim 0$ms & $\sim 1$s & $0.47 \pm 0.09$\\
	BAMCP (K = 10000, depth = 25, UGrid) & $\sim 0$ms & $\sim 1$s & $0.49 \pm 0.08$\\
	BAMCP (K = 10000, depth = 50, UGrid) & $\sim 0$ms & $\sim 1$s & $0.42 \pm 0.07$\\
	BAMCP (K = 25000, depth = 15, UGrid) & $\sim 0$ms & $\sim 3$s & $0.49 \pm 0.09$\\
	\textbf{BAMCP (K = 25000, depth = 25, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 3}$\textbf{s} & $\boldsymbol{0.51 \pm 0.09}$\\
	BAMCP (K = 25000, depth = 50, UGrid) & $\sim 0$ms & $\sim 3$s & $0.47 \pm 0.08$\\
	BFS3 (K = 1, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.3 \pm 0.07$\\
	BFS3 (K = 1, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.24 \pm 0.06$\\
	BFS3 (K = 1, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.28 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 2$ms & $0.33 \pm 0.07$\\
	BFS3 (K = 1, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 2$ms & $0.27 \pm 0.06$\\
	BFS3 (K = 1, C = 5, depth = 50, UGrid) & $\sim 0$ms & $\sim 5$ms & $0.28 \pm 0.06$\\
	BFS3 (K = 1, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 5$ms & $0.26 \pm 0.06$\\
	BFS3 (K = 1, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 8$ms & $0.31 \pm 0.06$\\
	BFS3 (K = 1, C = 10, depth = 50, UGrid) & $\sim 0$ms & $\sim 17$ms & $0.33 \pm 0.07$\\
	BFS3 (K = 1, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 10$ms & $0.36 \pm 0.08$\\
	BFS3 (K = 1, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 17$ms & $0.34 \pm 0.08$\\
	\textbf{BFS3 (K = 1, C = 15, depth = 50, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 32}$\textbf{ms} & $\boldsymbol{0.42 \pm 0.09}$\\
	BFS3 (K = 500, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 78$ms & $0.2 \pm 0.05$\\
	BFS3 (K = 500, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 154$ms & $0.25 \pm 0.06$\\
	BFS3 (K = 500, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 301$ms & $0.25 \pm 0.06$\\
	BFS3 (K = 500, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 127$ms & $0.23 \pm 0.06$\\
	BFS3 (K = 500, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 234$ms & $0.32 \pm 0.07$\\
	BFS3 (K = 500, C = 5, depth = 50, UGrid) & $\sim 0$ms & $\sim 506$ms & $0.28 \pm 0.06$\\
	BFS3 (K = 500, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 231$ms & $0.28 \pm 0.06$\\
	BFS3 (K = 500, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 376$ms & $0.29 \pm 0.06$\\
	BFS3 (K = 500, C = 10, depth = 50, UGrid) & $\sim 0$ms & $\sim 848$ms & $0.31 \pm 0.07$\\
	BFS3 (K = 500, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 296$ms & $0.3 \pm 0.06$\\
	BFS3 (K = 500, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 538$ms & $0.34 \pm 0.06$\\
	BFS3 (K = 500, C = 15, depth = 50, UGrid) & $\sim 0$ms & $\sim 1$s & $0.36 \pm 0.07$\\
	BFS3 (K = 1250, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 185$ms & $0.26 \pm 0.06$\\
	BFS3 (K = 1250, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 361$ms & $0.18 \pm 0.05$\\
	BFS3 (K = 1250, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 790$ms & $0.23 \pm 0.06$\\
	BFS3 (K = 1250, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 306$ms & $0.3 \pm 0.07$\\
	BFS3 (K = 1250, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 550$ms & $0.24 \pm 0.06$\\
	BFS3 (K = 1250, C = 5, depth = 50, UGrid) & $\sim 0$ms & $\sim 2$s & $0.27 \pm 0.06$\\
	BFS3 (K = 1250, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 471$ms & $0.32 \pm 0.07$\\
	BFS3 (K = 1250, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 928$ms & $0.31 \pm 0.06$\\
	BFS3 (K = 1250, C = 10, depth = 50, UGrid) & $\sim 0$ms & $\sim 2$s & $0.26 \pm 0.05$\\
	BFS3 (K = 1250, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 643$ms & $0.36 \pm 0.07$\\
	BFS3 (K = 1250, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 1$s & $0.3 \pm 0.06$\\
	BFS3 (K = 1250, C = 15, depth = 50, UGrid) & $\sim 0$ms & $\sim 3$s & $0.36 \pm 0.07$\\
	BFS3 (K = 2500, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 397$ms & $0.26 \pm 0.07$\\
	BFS3 (K = 2500, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 726$ms & $0.18 \pm 0.05$\\
	BFS3 (K = 2500, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 1$s & $0.24 \pm 0.06$\\
	BFS3 (K = 2500, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 543$ms & $0.26 \pm 0.06$\\
	BFS3 (K = 2500, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 1$s & $0.22 \pm 0.05$\\
	BFS3 (K = 2500, C = 5, depth = 50, UGrid) & $\sim 0$ms & $\sim 3$s & $0.26 \pm 0.06$\\
	BFS3 (K = 2500, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 684$ms & $0.36 \pm 0.07$\\
	BFS3 (K = 2500, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 2$s & $0.34 \pm 0.07$\\
	BFS3 (K = 2500, C = 10, depth = 50, UGrid) & $\sim 0$ms & $\sim 4$s & $0.35 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 883$ms & $0.33 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 2$s & $0.35 \pm 0.07$\\
	BFS3 (K = 2500, C = 15, depth = 50, UGrid) & $\sim 0$ms & $\sim 6$s & $0.4 \pm 0.08$\\
	BFS3 (K = 5000, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 782$ms & $0.23 \pm 0.05$\\
	BFS3 (K = 5000, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 1$s & $0.22 \pm 0.06$\\
	BFS3 (K = 5000, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 3$s & $0.31 \pm 0.07$\\
	BFS3 (K = 5000, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 834$ms & $0.23 \pm 0.05$\\
	BFS3 (K = 5000, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 2$s & $0.25 \pm 0.06$\\
	BFS3 (K = 5000, C = 5, depth = 50, UGrid) & $\sim 0$ms & $\sim 5$s & $0.22 \pm 0.05$\\
	BFS3 (K = 5000, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 989$ms & $0.37 \pm 0.07$\\
	BFS3 (K = 5000, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.33 \pm 0.07$\\
	BFS3 (K = 5000, C = 10, depth = 50, UGrid) & $\sim 0$ms & $\sim 7$s & $0.32 \pm 0.07$\\
	BFS3 (K = 5000, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 1$s & $0.35 \pm 0.07$\\
	BFS3 (K = 5000, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.36 \pm 0.07$\\
	BFS3 (K = 5000, C = 15, depth = 50, UGrid) & $\sim 0$ms & $\sim 9$s & $0.34 \pm 0.07$\\
	BFS3 (K = 10000, C = 2, depth = 15, UGrid) & $\sim 0$ms & $\sim 2$s & $0.18 \pm 0.05$\\
	BFS3 (K = 10000, C = 2, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.25 \pm 0.06$\\
	BFS3 (K = 10000, C = 2, depth = 50, UGrid) & $\sim 0$ms & $\sim 6$s & $0.23 \pm 0.05$\\
	BFS3 (K = 10000, C = 5, depth = 15, UGrid) & $\sim 0$ms & $\sim 2$s & $0.3 \pm 0.07$\\
	BFS3 (K = 10000, C = 5, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.27 \pm 0.06$\\
	BFS3 (K = 10000, C = 10, depth = 15, UGrid) & $\sim 0$ms & $\sim 1$s & $0.34 \pm 0.07$\\
	BFS3 (K = 10000, C = 10, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.33 \pm 0.07$\\
	BFS3 (K = 10000, C = 15, depth = 15, UGrid) & $\sim 0$ms & $\sim 1$s & $0.34 \pm 0.07$\\
	BFS3 (K = 10000, C = 15, depth = 25, UGrid) & $\sim 0$ms & $\sim 3$s & $0.39 \pm 0.08$\\
	SBOSS (epsilon = 1, delta = 9, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.08 \pm 0.04$\\
	SBOSS (epsilon = 1, delta = 7, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.08 \pm 0.03$\\
	SBOSS (epsilon = 1, delta = 5, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.15 \pm 0.05$\\
	SBOSS (epsilon = 1, delta = 3, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.16 \pm 0.05$\\
	SBOSS (epsilon = 1, delta = 1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.22 \pm 0.07$\\
	SBOSS (epsilon = 1, delta = 0.1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.18 \pm 0.06$\\
	SBOSS (epsilon = 1, delta = 0.01, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.17 \pm 0.06$\\
	SBOSS (epsilon = 1, delta = 0.001, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.17 \pm 0.06$\\
	SBOSS (epsilon = 0.1, delta = 9, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.08 \pm 0.04$\\
	SBOSS (epsilon = 0.1, delta = 7, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.07 \pm 0.04$\\
	SBOSS (epsilon = 0.1, delta = 5, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.09 \pm 0.03$\\
	SBOSS (epsilon = 0.1, delta = 3, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 0.1, delta = 1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 0.1, delta = 0.1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.17 \pm 0.05$\\
	SBOSS (epsilon = 0.1, delta = 0.01, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.25 \pm 0.07$\\
	SBOSS (epsilon = 0.1, delta = 0.001, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.24 \pm 0.07$\\
	SBOSS (epsilon = 0.01, delta = 9, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.07 \pm 0.03$\\
	SBOSS (epsilon = 0.01, delta = 7, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.09 \pm 0.04$\\
	SBOSS (epsilon = 0.01, delta = 5, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.1 \pm 0.04$\\
	SBOSS (epsilon = 0.01, delta = 3, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.15 \pm 0.05$\\
	SBOSS (epsilon = 0.01, delta = 1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.16 \pm 0.05$\\
	SBOSS (epsilon = 0.01, delta = 0.1, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.23 \pm 0.07$\\
	SBOSS (epsilon = 0.01, delta = 0.01, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 0.01, delta = 0.001, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.15 \pm 0.05$\\
	SBOSS (epsilon = 0.001, delta = 9, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.09 \pm 0.05$\\
	SBOSS (epsilon = 0.001, delta = 7, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.09 \pm 0.05$\\
	SBOSS (epsilon = 0.001, delta = 5, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.11 \pm 0.04$\\
	SBOSS (epsilon = 0.001, delta = 3, UGrid) & $\sim 0$ms & $\sim 0$ms & $0.15 \pm 0.05$\\
	SBOSS (epsilon = 0.001, delta = 1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.22 \pm 0.06$\\
	\textbf{SBOSS (epsilon = 0.001, delta = 0.1, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 2}$\textbf{ms} & $\boldsymbol{0.29 \pm 0.07}$\\
	SBOSS (epsilon = 0.001, delta = 0.01, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.2 \pm 0.06$\\
	SBOSS (epsilon = 0.001, delta = 0.001, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.21 \pm 0.06$\\
	SBOSS (epsilon = 0.0001, delta = 0.0001, UGrid) & $\sim 0$ms & $\sim 13$ms & $0.21 \pm 0.06$\\
	SBOSS (epsilon = 0.0001, delta = 1e-05, UGrid) & $\sim 0$ms & $\sim 15$ms & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 0.0001, delta = 1e-06, UGrid) & $\sim 0$ms & $\sim 15$ms & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 1e-05, delta = 0.0001, UGrid) & $\sim 0$ms & $\sim 181$ms & $0.24 \pm 0.07$\\
	SBOSS (epsilon = 1e-05, delta = 1e-05, UGrid) & $\sim 0$ms & $\sim 170$ms & $0.22 \pm 0.06$\\
	SBOSS (epsilon = 1e-05, delta = 1e-06, UGrid) & $\sim 0$ms & $\sim 154$ms & $0.16 \pm 0.05$\\
	SBOSS (epsilon = 1e-06, delta = 0.0001, UGrid) & $\sim 0$ms & $\sim 2$s & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 1e-06, delta = 1e-05, UGrid) & $\sim 0$ms & $\sim 2$s & $0.19 \pm 0.06$\\
	SBOSS (epsilon = 1e-06, delta = 1e-06, UGrid) & $\sim 0$ms & $\sim 2$s & $0.21 \pm 0.06$\\
	\textbf{BEB (beta = 0.25, UGrid)} & $\boldsymbol{\sim 0}$\textbf{ms} & $\boldsymbol{\sim 1}$\textbf{ms} & $\boldsymbol{0.29 \pm 0.05}$\\
	BEB (beta = 0.5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.24 \pm 0.04$\\
	BEB (beta = 1, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.23 \pm 0.05$\\
	BEB (beta = 1.5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.25 \pm 0.05$\\
	BEB (beta = 2, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.25 \pm 0.04$\\
	BEB (beta = 2.5, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.22 \pm 0.04$\\
	BEB (beta = 3, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.22 \pm 0.04$\\
	BEB (beta = 4, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.28 \pm 0.05$\\
	BEB (beta = 8, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.27 \pm 0.04$\\
	BEB (beta = 16, UGrid) & $\sim 0$ms & $\sim 1$ms & $0.25 \pm 0.05$\\
\end{longtable}

